Implications of LHCb measurements and future prospects

During 2011 the LHCb experiment at CERN collected 1.0 fb-1 of sqrt{s} = 7 TeV pp collisions. Due to the large heavy quark production cross-sections, these data provide unprecedented samples of heavy flavoured hadrons. The first results from LHCb have made a significant impact on the flavour physics landscape and have definitively proved the concept of a dedicated experiment in the forward region at a hadron collider. This document discusses the implications of these first measurements on classes of extensions to the Standard Model, bearing in mind the interplay with the results of searches for on-shell production of new particles at ATLAS and CMS. The physics potential of an upgrade to the LHCb detector, which would allow an order of magnitude more data to be collected, is emphasised.

==> LHCb_authorlist_FTDR.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\centerline{\large\bf The LHCb collaboration}
\begin{flushleft}
\small
I.~Bediaga$^{1}$, 
J.M.~De~Miranda$^{1}$, 
F.~Ferreira~Rodrigues$^{1}$, 
J.~Magnin$^{1}$, 
A.~Massafferri$^{1}$, 
I.~Nasteva$^{1}$, 
A.C.~dos~Reis$^{1}$\newline{\it
$ ^{1}$Centro Brasileiro de Pesquisas F\'{i}sicas (CBPF), Rio de Janeiro, Brazil}\\[2ex]
S.~Amato$^{2}$, 
K.~Carvalho~Akiba$^{2}$, 
L.~De~Paula$^{2}$, 
O.~Francisco$^{2}$, 
M.~Gandelman$^{2}$, 
A.~Gomes$^{2}$, 
J.H.~Lopes$^{2}$, 
J.M.~Otalora~Goicochea$^{2}$, 
E.~Polycarpo$^{2}$, 
M.S.~Rangel$^{2}$, 
B.~Souza~De~Paula$^{2}$, 
D.~Vieira$^{2}$\newline{\it
$ ^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil}\\[2ex]
C.~G\"{o}bel$^{3}$, 
J.~Molina~Rodriguez$^{3}$\newline{\it
$ ^{3}$Pontif\'{i}cia Universidade Cat\'{o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil}\\[2ex]
P.~Chen$^{4,39}$, 
Y.~Gao$^{4}$, 
G.~Gong$^{4}$, 
H.~Gong$^{4}$, 
F.~Jing$^{4}$, 
L.~Li$^{4}$, 
Y.~Li$^{4}$, 
B.~Liu$^{4}$, 
H.~Lu$^{4}$, 
B.~Shao$^{4}$, 
S.~Wu$^{4}$, 
T.~Xue$^{4}$, 
Z.~Yang$^{4}$, 
X.~Yuan$^{4}$, 
M.~Zeng$^{4}$, 
F.~Zhang$^{4}$, 
Y.~Zhang$^{4}$, 
L.~Zhong$^{4}$\newline{\it
$ ^{4}$Center for High Energy Physics, Tsinghua University, Beijing, China}\\[2ex]
I.~De~Bonis$^{5}$, 
D.~Decamp$^{5}$, 
C.~Drancourt$^{5}$, 
Ph.~Ghez$^{5}$, 
P.~Hopchev$^{5}$, 
J.-P.~Lees$^{5}$, 
I.V.~Machikhiliyan$^{5,31}$, 
M.-N.~Minard$^{5}$, 
B.~Pietrzyk$^{5}$, 
S.~T'Jampens$^{5}$, 
V.~Tisserand$^{5}$, 
E.~Tournefier$^{5,53}$, 
G.~Vouters$^{5}$\newline{\it
$ ^{5}$LAPP, Universit\'{e} de Savoie, CNRS/IN2P3, Annecy-Le-Vieux, France}\\[2ex]
Z.~Ajaltouni$^{6}$, 
H.~Chanal$^{6}$, 
E.~Cogneras$^{6}$, 
O.~Deschamps$^{6}$, 
I.~El~Rifai$^{6}$, 
P.~Henrard$^{6}$, 
M.~Hoballah$^{6}$, 
M.~Jahjah~Hussein$^{6}$, 
R.~Lef\`{e}vre$^{6}$, 
L.~Li~Gioi$^{6}$, 
S.~Monteil$^{6}$, 
V.~Niess$^{6}$, 
P.~Perret$^{6}$, 
D.A.~Roa~Romero$^{6}$, 
K.~Sobczak$^{6}$\newline{\it
$ ^{6}$Clermont Universit\'{e}, Universit\'{e} Blaise Pascal, CNRS/IN2P3, LPC, Clermont-Ferrand, France}\\[2ex]
C.~Adrover$^{7}$, 
E.~Aslanides$^{7}$, 
J.-P.~Cachemiche$^{7}$, 
J.~Cogan$^{7}$, 
P.-Y.~Duval$^{7}$, 
F.~Hachon$^{7}$, 
B.~Khanji$^{7}$, 
R.~Le~Gac$^{7}$, 
O.~Leroy$^{7}$, 
G.~Mancinelli$^{7}$, 
E.~Maurice$^{7}$, 
M.~Perrin-Terrin$^{7}$, 
F.~Rethore$^{7}$, 
M.~Sapunov$^{7}$, 
J.~Serrano$^{7}$, 
A.~Tsaregorodtsev$^{7}$\newline{\it
$ ^{7}$CPPM, Aix-Marseille Universit\'{e}, CNRS/IN2P3, Marseille, France}\\[2ex]
S.~Barsuk$^{8}$, 
C.~Beigbeder-Beau$^{8}$, 
T.~Cac\'{e}r\`{e}s$^{8}$, 
O.~Callot$^{8}$, 
D.~Charlet$^{8}$, 
O.~Duarte$^{8}$, 
J.~He$^{8}$, 
B.~Jean-Marie$^{8}$, 
O.~Kochebina$^{8}$, 
J.~Lefran\c{c}ois$^{8}$, 
F.~Machefert$^{8}$, 
A.~Mart\'{i}n~S\'{a}nchez$^{8}$, 
M.~Nicol$^{8}$, 
P.~Robbe$^{8}$, 
M.-H.~Schune$^{8}$, 
M.~Teklishyn$^{8}$, 
V.~Tocut$^{8}$, 
B.~Viaud$^{8}$, 
I.~Videau$^{8}$\newline{\it
$ ^{8}$LAL, Universit\'{e} Paris-Sud, CNRS/IN2P3, Orsay, France}\\[2ex]
E.~Ben-Haim$^{9}$, 
M.~Benayoun$^{9}$, 
P.~David$^{9}$, 
L.~Del~Buono$^{9}$, 
A.~Martens$^{9}$, 
F.~Polci$^{9}$\newline{\it
$ ^{9}$LPNHE, Universit\'{e} Pierre et Marie Curie, Universit\'{e} Paris Diderot, CNRS/IN2P3, Paris, France}\\[2ex]
T.~Brambach$^{10}$, 
Ch.~Cauet$^{10}$, 
M.~Deckenhoff$^{10}$, 
M.~Domke$^{10}$, 
R.~Ekelhof$^{10}$, 
M.~Kaballo$^{10}$, 
T.M.~Karbach$^{10}$, 
F.~Kruse$^{10}$, 
J.~Merkel$^{10}$, 
K.~Rudloff$^{10}$, 
S.~Schleich$^{10}$, 
M.~Schlupp$^{10}$, 
B.~Spaan$^{10}$, 
S.~Swientek$^{10}$, 
K.~Warda$^{10}$, 
J.~Wishahi$^{10}$\newline{\it
$ ^{10}$Fakult\"{a}t Physik, Technische Universit\"{a}t Dortmund, Dortmund, Germany}\\[2ex]
C.~Bauer$^{11}$, 
M.~Britsch$^{11}$, 
C.~F\"{o}hr$^{11}$, 
M.~Fontana$^{11}$, 
H.~Fuchs$^{11}$, 
W.~Hofmann$^{11}$, 
T.~Kihm$^{11}$, 
D.~Popov$^{11}$, 
M.~Schmelling$^{11}$, 
D.~Volyanskyy$^{11}$, 
H.~Voss$^{11}$, 
M.~Zavertyaev$^{11,a}$\newline{\it
$ ^{11}$Max-Planck-Institut f\"{u}r Kernphysik (MPIK), Heidelberg, Germany}\\[2ex]
S.~Bachmann$^{12}$, 
A.~Bien$^{12}$, 
J.~Blouw$^{12}$, 
F.~Dordei$^{12}$, 
C.~F\"{a}rber$^{12}$, 
E.~Gersabeck$^{12}$, 
S.~Hansmann-Menzemer$^{12}$, 
A.~Jaeger$^{12}$, 
K.~Kreplin$^{12}$, 
G.~Krocker$^{12}$, 
C.~Linn$^{12}$, 
J.~Marks$^{12}$, 
M.~Meissner$^{12}$, 
T.~Nikodem$^{12}$, 
P.~Seyfert$^{12}$, 
S.~Stahl$^{12}$, 
J.~van~Tilburg$^{12}$, 
U.~Uwer$^{12}$, 
S.~Wandernoth$^{12}$, 
D.~Wiedner$^{12}$, 
A.~Zhelezov$^{12}$\newline{\it
$ ^{12}$Physikalisches Institut, Ruprecht-Karls-Universit\"{a}t Heidelberg, Heidelberg, Germany}\\[2ex]
O.~Gr\"{u}nberg$^{13}$, 
T.~Hartmann$^{13}$, 
C.~Vo\ss$^{13}$, 
R.~Waldi$^{13}$\newline{\it
$ ^{13}$Institut f\"{u}r Physik, Universit\"{a}t Rostock, Rostock, Germany}\\[2ex]
S.~Bifani$^{14}$, 
S.~Farry$^{14}$, 
P.~Ilten$^{14}$, 
T.~Kechadi$^{14}$, 
Z.~Mathe$^{14}$, 
R.~McNulty$^{14}$, 
R.~Wallace$^{14}$, 
W.C.~Zhang$^{14}$\newline{\it
$ ^{14}$School of Physics, University College Dublin, Dublin, Ireland}\\[2ex]
D.A.~Milanes$^{15}$, 
A.~Palano$^{15,b}$\newline{\it
$ ^{15}$Sezione INFN di Bari, Bari, Italy}\\[2ex]
A.~Carbone$^{16,c}$, 
I.~D'Antone$^{16}$, 
D.~Derkach$^{16,38}$, 
A.~Falabella$^{16,e}$, 
D.~Galli$^{16,c}$, 
I.~Lax$^{16}$, 
U.~Marconi$^{16}$, 
S.~Perazzini$^{16,c}$, 
V.~Vagnoni$^{16}$, 
G.~Valenti$^{16}$, 
M.~Zangoli$^{16}$\newline{\it
$ ^{16}$Sezione INFN di Bologna, Bologna, Italy}\\[2ex]
W.~Bonivento$^{17}$, 
S.~Cadeddu$^{17}$, 
A.~Cardini$^{17}$, 
A.~Lai$^{17}$, 
G.~Manca$^{17,d}$, 
R.~Oldeman$^{17,d,38}$, 
B.~Saitta$^{17,d}$\newline{\it
$ ^{17}$Sezione INFN di Cagliari, Cagliari, Italy}\\[2ex]
W.~Baldini$^{18}$, 
C.~Bozzi$^{18}$, 
F.~Evangelisti$^{18}$, 
L.~Landi$^{18,e}$, 
A.~Mazurov$^{18,33,38}$, 
M.~Savrie$^{18,e}$, 
S.~Squerzanti$^{18}$, 
S.~Vecchi$^{18}$\newline{\it
$ ^{18}$Sezione INFN di Ferrara, Ferrara, Italy}\\[2ex]
A.~Bizzeti$^{19,h}$, 
M.~Frosini$^{19,f}$, 
G.~Graziani$^{19}$, 
G.~Passaleva$^{19}$, 
M.~Veltri$^{19,g}$\newline{\it
$ ^{19}$Sezione INFN di Firenze, Firenze, Italy}\\[2ex]
M.~Anelli$^{20}$, 
F.~Archilli$^{20,38}$, 
G.~Bencivenni$^{20}$, 
P.~Campana$^{20,38}$, 
P.~Ciambrone$^{20}$, 
P.~De~Simone$^{20}$, 
G.~Felici$^{20}$, 
G.~Lanfranchi$^{20,38}$, 
M.~Palutan$^{20}$, 
A.~Saputi$^{20}$, 
A.~Sarti$^{20,l}$, 
B.~Sciascia$^{20}$, 
F.~Soomro$^{20,38}$\newline{\it
$ ^{20}$Laboratori Nazionali dell'INFN di Frascati, Frascati, Italy}\\[2ex]
R.~Cardinale$^{21,i,38}$, 
F.~Fontanelli$^{21,i}$, 
C.~Patrignani$^{21,i}$, 
A.~Petrolini$^{21,i}$\newline{\it
$ ^{21}$Sezione INFN di Genova, Genova, Italy}\\[2ex]
M.~Calvi$^{22,j}$, 
S.~Furcas$^{22}$, 
A.~Giachero$^{22}$, 
C.~Gotti$^{22}$, 
M.~Kucharczyk$^{22,26,38,j}$, 
M.~Maino$^{22}$, 
C.~Matteuzzi$^{22}$, 
G.~Pessina$^{22}$\newline{\it
$ ^{22}$Sezione INFN di Milano Bicocca, Milano, Italy}\\[2ex]
G.~Carboni$^{23,k}$, 
S.~De~Capua$^{23,k}$, 
G.~Sabatino$^{23,k}$, 
E.~Santovetti$^{23,k}$, 
A.~Satta$^{23}$\newline{\it
$ ^{23}$Sezione INFN di Roma Tor Vergata, Roma, Italy}\\[2ex]
A.A.~Alves~Jr$^{24}$, 
G.~Auriemma$^{24,m}$, 
V.~Bocci$^{24}$, 
G.~Martellotti$^{24}$, 
G.~Penso$^{24,l}$, 
D.~Pinci$^{24}$, 
R.~Santacesaria$^{24}$, 
C.~Satriano$^{24,m}$, 
A.~Sciubba$^{24}$\newline{\it
$ ^{24}$Sezione INFN di Roma La Sapienza, Roma, Italy}\\[2ex]
S.~Nisar$^{25}$\newline{\it
$ ^{25}$Institute of Information Technology, COMSATS, Lahore, Pakistan}\\[2ex]
P.~Morawski$^{26}$, 
G.~Polok$^{26}$, 
M.~Witek$^{26}$\newline{\it
$ ^{26}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak\'{o}w, Poland}\\[2ex]
B.~Muryn$^{27}$, 
A.~Oblakowska-Mucha$^{27}$, 
K.~Senderowska$^{27}$, 
T.~Szumlak$^{27}$\newline{\it
$ ^{27}$AGH University of Science and Technology, Krak\'{o}w, Poland}\\[2ex]
Z.~Guzik$^{28}$, 
A.~Nawrot$^{28}$, 
M.~Szczekowski$^{28}$, 
A.~Ukleja$^{28}$\newline{\it
$ ^{28}$Soltan Institute for Nuclear Studies, Warsaw, Poland}\\[2ex]
I.~Burducea$^{29}$, 
C.~Coca$^{29}$, 
M.~Dogaru$^{29}$, 
A.~Grecu$^{29}$, 
F.~Maciuc$^{29}$, 
R.~Muresan$^{29}$, 
M.~Orlandea$^{29}$, 
C.~Pavel-Nicorescu$^{29}$, 
B.~Popovici$^{29}$, 
S.~Stoica$^{29}$, 
M.~Straticiuc$^{29}$, 
E.~Teodorescu$^{29}$\newline{\it
$ ^{29}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania}\\[2ex]
G.~Alkhazov$^{30}$, 
B.~Bochin$^{30}$, 
N.~Bondar$^{30}$, 
A.~Dzyuba$^{30}$, 
S.~Gets$^{30}$, 
V.~Golovtsov$^{30}$, 
A.~Kashchuk$^{30}$, 
O.~Maev$^{30,38}$, 
M.~Matveev$^{30}$, 
N.~Sagidova$^{30}$, 
Y.~Shcheglov$^{30}$, 
S.~Volkov$^{30}$, 
A.~Vorobyev$^{30}$\newline{\it
$ ^{30}$Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia}\\[2ex]
V.~Balagura$^{31}$, 
S.~Belogurov$^{31}$, 
I.~Belyaev$^{31}$, 
V.~Egorychev$^{31}$, 
D.~Golubkov$^{31}$, 
T.~Kvaratskheliya$^{31,38}$, 
D.~Savrina$^{31}$, 
A.~Semennikov$^{31}$, 
P.~Shatalov$^{31}$, 
V.~Shevchenko$^{31}$, 
A.~Zhokhov$^{31}$\newline{\it
$ ^{31}$Institute of Theoretical and Experimental Physics (ITEP), Moscow, Russia}\\[2ex]
A.~Berezhnoy$^{32}$, 
G.~Bogdanova$^{32}$, 
I.~Komarov$^{32}$, 
M.~Korolev$^{32}$, 
A.~Leflat$^{32,38}$, 
N.~Nikitin$^{32}$, 
V.~Volkov$^{32}$, 
E.~Zverev$^{32}$\newline{\it
$ ^{32}$Institute of Nuclear Physics, Moscow State University (SINP MSU), Moscow, Russia}\\[2ex]
S.~Filippov$^{33}$, 
E.~Gushchin$^{33}$, 
O.~Karavichev$^{33}$, 
L.~Kravchuk$^{33}$, 
Y.~Kudenko$^{33}$, 
S.~Laptev$^{33}$, 
A.~Tikhonov$^{33}$\newline{\it
$ ^{33}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAN), Moscow, Russia}\\[2ex]
A.~Bondar$^{34}$, 
S.~Eidelman$^{34}$, 
P.~Krokovny$^{34}$, 
V.~Kudryavtsev$^{34}$, 
L.~Shekhtman$^{34}$, 
V.~Vorobyev$^{34}$\newline{\it
$ ^{34}$Budker Institute of Nuclear Physics (SB RAS) and Novosibirsk State University, Novosibirsk, Russia}\\[2ex]
A.~Artamonov~$^{35}$, 
K.~Belous$^{35}$, 
R.~Dzhelyadin$^{35}$, 
Yu.~Guz$^{35}$, 
A.~Likhoded$^{35}$, 
A.~Novoselov$^{35}$, 
V.~Obraztsov$^{35}$, 
A.~Ostankov$^{35}$, 
V.~Romanovsky$^{35}$, 
M.~Shapkin$^{35}$, 
O.~Stenyakin$^{35}$, 
O.~Yushchenko$^{35}$\newline{\it
$ ^{35}$Institute for High Energy Physics (IHEP), Protvino, Russia}\\[2ex]
C.~Abellan~Beteta$^{36,n}$, 
M.~Calvo~Gomez$^{36,n}$, 
A.~Camboni$^{36}$, 
A.~Casajus~Ramo$^{36}$, 
A.~Comerma-Montells$^{36}$, 
F.~Domingo~Bonal$^{36,n}$, 
L.~Garrido$^{36}$, 
D.~Gascon$^{36}$, 
M.~Grabalosa~G\'{a}ndara$^{36}$, 
R.~Graciani~Diaz$^{36}$, 
E.~Graug\'{e}s$^{36}$, 
E.~Lopez~Asamar$^{36}$, 
J.~Mauricio$^{36}$, 
V.~Mendez-Munoz$^{36,o}$, 
A.~P\'{e}rez-Calero~Yzquierdo$^{36}$, 
E.~Picatoste~Olloqui$^{36}$, 
B.~Pie~Valls$^{36}$, 
C.~Potterat$^{36}$, 
A.~Puig~Navarro$^{36}$, 
M.~Rosello$^{36,n}$, 
H.~Ruiz$^{36}$, 
R.~Vazquez~Gomez$^{36}$, 
X.~Vilasis-Cardona$^{36,n}$\newline{\it
$ ^{36}$Universitat de Barcelona, Barcelona, Spain}\\[2ex]
B.~Adeva$^{37}$, 
P.~Alvarez~Cartelle$^{37}$, 
X.~Cid~Vidal$^{37}$, 
A.~Dosil~Su\'{a}rez$^{37}$, 
D.~Esperante~Pereira$^{37}$, 
V.~Fernandez~Albor$^{37}$, 
A.~Gallas~Torreira$^{37}$, 
J.A.~Hernando~Morata$^{37}$, 
A.~Pazos~Alvarez$^{37}$, 
E.~Perez~Trigo$^{37}$, 
M.~Plo~Casasus$^{37}$, 
P.~Rodriguez~Perez$^{37}$, 
J.J.~Saborido~Silva$^{37}$, 
B.~Sanmartin~Sedes$^{37}$, 
C.~Santamarina~Rios$^{37}$, 
M.~Seco$^{37}$, 
P.~Vazquez~Regueiro$^{37}$, 
J.~Visniakov$^{37}$\newline{\it
$ ^{37}$Universidad de Santiago de Compostela, Santiago de Compostela, Spain}\\[2ex]
J.~Albrecht$^{38}$, 
F.~Alessio$^{38}$, 
C.~Barschel$^{38}$, 
T.~Blake$^{38}$, 
E.~Bonaccorsi$^{38}$, 
L.~Brarda$^{38}$, 
J.~Buytaert$^{38}$, 
M.~Cattaneo$^{38}$, 
B.~Chadaj$^{38}$, 
Ph.~Charpentier$^{38}$, 
M.~Chebbi$^{38}$, 
K.~Ciba$^{38}$, 
M.~Clemencic$^{38}$, 
J.~Closier$^{38}$, 
P.~Collins$^{38}$, 
B.~Corajod$^{38}$, 
G.~Corti$^{38}$, 
B.~Couturier$^{38}$, 
C.~D'Ambrosio$^{38}$, 
G.~Decreuse$^{38}$, 
H.~Dijkstra$^{38}$, 
R.~Dumps$^{38}$, 
M.~Ferro-Luzzi$^{38}$, 
R.~Forty$^{38}$, 
C.~Fournier$^{38}$, 
M.~Frank$^{38}$, 
C.~Frei$^{38}$, 
C.~Gaspar$^{38}$, 
M.~Gersabeck$^{38}$, 
V.V.~Gligorov$^{38}$, 
L.A.~Granado~Cardoso$^{38}$, 
T.~Gys$^{38}$, 
C.~Haen$^{38}$, 
E.~van~Herwijnen$^{38}$, 
R.~Jacobsson$^{38}$, 
O.~Jamet$^{38}$, 
B.~Jost$^{38}$, 
M.~Karacson$^{38}$, 
R.~Kristic$^{38}$, 
D.~Lacarrere$^{38}$, 
E.~Lanciotti$^{38}$, 
C.~Langenbruch$^{38}$, 
R.~Lindner$^{38}$, 
G.~Liu$^{38}$, 
D.~Martinez~Santos$^{38}$, 
R.~Matev$^{38}$, 
N.~Neufeld$^{38}$, 
J.~Panman$^{38}$, 
M.~Pepe~Altarelli$^{38}$, 
D.~Piedigrossi$^{38}$, 
N.~Rauschmayr$^{38}$, 
S.~Roiser$^{38}$, 
L.~Roy$^{38}$, 
T.~Ruf$^{38}$, 
H.~Schindler$^{38}$, 
B.~Schmidt$^{38}$, 
T.~Schneider$^{38}$, 
A.~Schopper$^{38}$, 
R.~Schwemmer$^{38}$, 
F.~Stagni$^{38}$, 
V.K.~Subbiah$^{38}$, 
F.~Teubert$^{38}$, 
E.~Thomas$^{38}$, 
D.~Tonelli$^{38}$, 
M.~Ubeda~Garcia$^{38}$, 
O.~Ullaland$^{38}$, 
M.~Vesterinen$^{38}$, 
J.~Wicht$^{38}$, 
W.~Witzeling$^{38}$, 
K.~Wyllie$^{38}$, 
A.~Zvyagin$^{38}$\newline{\it
$ ^{38}$European Organization for Nuclear Research (CERN), Geneva, Switzerland}\\[2ex]
Y.~Amhis$^{39}$, 
A.~Bay$^{39}$, 
F.~Bernard$^{39}$, 
F.~Blanc$^{39}$, 
J.~Bressieux$^{39}$, 
G.A.~Cowan$^{39}$, 
H.~Degaudenzi$^{39,38}$, 
F.~Dupertuis$^{39}$, 
V.~Fave$^{39}$, 
R.~Frei$^{39}$, 
N.~Gauvin$^{39}$, 
G.~Haefeli$^{39}$, 
P.~Jaton$^{39}$, 
A.~Keune$^{39}$, 
M.~Knecht$^{39}$, 
V.N.~La~Thi$^{39}$, 
N.~Lopez-March$^{39}$, 
J.~Luisier$^{39}$, 
R.~M\"{a}rki$^{39}$, 
B.~Muster$^{39}$, 
T.~Nakada$^{39}$, 
A.D.~Nguyen$^{39}$, 
C.~Nguyen-Mau$^{39,p}$, 
J.~Prisciandaro$^{39}$, 
B.~Rakotomiaramanana$^{39}$, 
J.~Rouvinet$^{39}$, 
O.~Schneider$^{39}$, 
P.~Szczypka$^{39}$, 
S.~Tourneur$^{39}$, 
M.T.~Tran$^{39}$, 
G.~Veneziano$^{39}$\newline{\it
$ ^{39}$Ecole Polytechnique F\'{e}d\'{e}rale de Lausanne (EPFL), Lausanne, Switzerland}\\[2ex]
J.~Anderson$^{40}$, 
R.~Bernet$^{40}$, 
A.~B\"{u}chler-Germann$^{40}$, 
A.~Bursche$^{40}$, 
N.~Chiapolini$^{40}$, 
M.~De~Cian$^{40}$, 
Ch.~Elsasser$^{40}$, 
K.~M\"{u}ller$^{40}$, 
J.~Palacios$^{40}$, 
C.~Salzmann$^{40}$, 
S.~Saornil~Gamarra$^{40}$, 
N.~Serra$^{40}$, 
O.~Steinkamp$^{40}$, 
U.~Straumann$^{40}$, 
M.~Tobin$^{40}$, 
A.~Vollhardt$^{40}$\newline{\it
$ ^{40}$Physik-Institut, Universit\"{a}t Z\"{u}rich, Z\"{u}rich, Switzerland}\\[2ex]
R.~Aaij$^{41}$, 
S.~Ali$^{41}$, 
H.~Band$^{41}$, 
Th.~Bauer$^{41}$, 
M.~van~Beuzekom$^{41}$, 
V.~van~Beveren$^{41}$, 
H.~Boer~Rookhuizen$^{41}$, 
L.~Ceelie$^{41}$, 
V.~Coco$^{41}$, 
P.N.Y.~David$^{41}$, 
K.~De~Bruyn$^{41}$, 
P.~De~Groen$^{41}$, 
D.~van~Eijk$^{41}$, 
C.~Farinelli$^{41}$, 
V.~Gromov$^{41}$, 
B.~van~der~Heijden$^{41}$, 
V.~Heijne$^{41}$, 
W.~Hulsbergen$^{41}$, 
E.~Jans$^{41}$, 
F.~Jansen$^{41}$, 
L.~Jansen$^{41}$, 
P.~Jansweijer$^{41}$, 
R.~Kluit$^{41}$, 
P.~Koppenburg$^{41}$, 
A.~Kozlinskiy$^{41}$, 
J.~van~Leerdam$^{41}$, 
M.~Martinelli$^{41}$, 
M.~Merk$^{41}$, 
I.~Mous$^{41}$, 
B.~Munneke$^{41}$, 
S.~Oggero$^{41}$, 
M.~van~Overbeek$^{41}$, 
A.~Pellegrino$^{41}$, 
O.~van~Petten$^{41}$, 
E.~Roeland$^{41}$, 
K.~de~Roo$^{41}$, 
A.~Schimmel$^{41}$, 
H.~Schuijlenburg$^{41}$, 
T.~Sluijk$^{41}$, 
B.~Storaci$^{41}$, 
P.~Tsopelas$^{41}$, 
N.~Tuning$^{41}$, 
W.~Vink$^{41}$, 
P.~Wenerke$^{41}$, 
L.~Wiggers$^{41}$, 
F.~Zappon$^{41}$, 
A.~Zwart$^{41}$\newline{\it
$ ^{41}$Nikhef National Institute for Subatomic Physics, Amsterdam, The Netherlands}\\[2ex]
J.~van~den~Brand$^{42}$, 
F.~Dettori$^{42}$, 
T.~Ketel$^{42}$, 
R.F.~Koopman$^{42}$, 
J.~Kos$^{42}$, 
R.W.~Lambert$^{42}$, 
F.~Mul$^{42}$, 
G.~Raven$^{42}$, 
M.~Schiller$^{42}$, 
S.~Tolk$^{42}$\newline{\it
$ ^{42}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, The Netherlands}\\[2ex]
A.~Dovbnya$^{43}$, 
S.~Kandybei$^{43}$, 
I.~Raniuk$^{43}$, 
I.~Shapoval$^{43,38}$, 
O.~Shevchenko$^{43}$\newline{\it
$ ^{43}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine}\\[2ex]
V.~Iakovenko$^{44}$, 
Y.~Nikolaiko$^{44}$, 
O.~Okhrimenko$^{44}$, 
M.~Pugatch$^{44}$, 
V.~Pugatch$^{44}$\newline{\it
$ ^{44}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine}\\[2ex]
P.J.W.~Faulkner$^{45}$, 
I.R.~Kenyon$^{45}$, 
C.~Lazzeroni$^{45}$, 
J.~McCarthy$^{45}$, 
M.W.~Slater$^{45}$, 
N.K.~Watson$^{45}$\newline{\it
$ ^{45}$University of Birmingham, Birmingham, United Kingdom}\\[2ex]
M.~Adinolfi$^{46}$, 
J.~Benton$^{46}$, 
N.H.~Brook$^{46}$, 
A.~Cook$^{46}$, 
M.~Coombes$^{46}$, 
T.~Hampson$^{46}$, 
S.T.~Harnew$^{46}$, 
P.~Naik$^{46}$, 
J.H.~Rademacker$^{46}$, 
A.~Solomin$^{46}$, 
D.~Souza$^{46}$, 
J.J.~Velthuis$^{46}$, 
D.~Voong$^{46}$\newline{\it
$ ^{46}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom}\\[2ex]
W.~Barter$^{47}$, 
M.-O.~Bettler$^{47}$, 
H.V.~Cliff$^{47}$, 
J.~Garra~Tico$^{47}$, 
V.~Gibson$^{47}$, 
S.~Gregson$^{47}$, 
S.C.~Haines$^{47}$, 
C.R.~Jones$^{47}$, 
S.~Sigurdsson$^{47}$, 
D.R.~Ward$^{47}$, 
S.A.~Wotton$^{47}$, 
S.~Wright$^{47}$\newline{\it
$ ^{47}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom}\\[2ex]
J.J.~Back$^{48}$, 
D.~Craik$^{48}$, 
D.~Dossett$^{48}$, 
T.~Gershon$^{48,38}$, 
M.~Kreps$^{48}$, 
T.~Latham$^{48}$, 
T.~Pila\v{r}$^{48}$, 
A.~Poluektov$^{48,34}$, 
M.M.~Reid$^{48}$, 
R.~Silva~Coutinho$^{48}$, 
M.~Whitehead$^{48}$, 
M.P.~Williams$^{48,49}$\newline{\it
$ ^{48}$Department of Physics, University of Warwick, Coventry, United Kingdom}\\[2ex]
S.~Easo$^{49}$, 
R.~Nandakumar$^{49}$, 
A.~Papanestis$^{49}$, 
G.N.~Patrick$^{49}$, 
S.~Ricciardi$^{49}$, 
F.F.~Wilson$^{49}$\newline{\it
$ ^{49}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom}\\[2ex]
S.~Benson$^{50}$, 
P.E.L.~Clarke$^{50}$, 
R.~Currie$^{50}$, 
S.~Eisenhardt$^{50}$, 
C.~Fitzpatrick$^{50}$, 
D.~Lambert$^{50}$, 
H.~Luo$^{50}$, 
H.~Mejia$^{50}$, 
F.~Muheim$^{50}$, 
M.~Needham$^{50}$, 
S.~Playfer$^{50}$, 
A.~Sparkes$^{50}$, 
Y.~Xie$^{50}$\newline{\it
$ ^{50}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom}\\[2ex]
M.~Alexander$^{51}$, 
J.~Beddow$^{51}$, 
S.~Borghi$^{51,54}$, 
L.~Eklund$^{51}$, 
D.~Hynds$^{51}$, 
S.~Ogilvy$^{51}$, 
M.~Pappagallo$^{51}$, 
E.~Rodrigues$^{51,54}$, 
P.~Sail$^{51}$, 
F.J.P.~Soler$^{51}$, 
P.~Spradlin$^{51}$\newline{\it
$ ^{51}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom}\\[2ex]
T.J.V.~Bowcock$^{52}$, 
H.~Brown$^{52}$, 
G.~Casse$^{52}$, 
S.~Donleavy$^{52}$, 
K.~Hennessy$^{52}$, 
E.~Hicks$^{52}$, 
T.~Huse$^{52}$, 
D.~Hutchcroft$^{52}$, 
M.~Liles$^{52}$, 
G.D.~Patel$^{52}$, 
K.~Rinnert$^{52}$, 
T.~Shears$^{52}$, 
N.A.~Smith$^{52}$\newline{\it
$ ^{52}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom}\\[2ex]
L.~Carson$^{53}$, 
G.~Ciezarek$^{53}$, 
S.~Cunliffe$^{53}$, 
U.~Egede$^{53}$, 
A.~Golutvin$^{53,31,38}$, 
S.~Hall$^{53}$, 
P.~Owen$^{53}$, 
C.J.~Parkinson$^{53}$, 
M.~Patel$^{53}$, 
K.~Petridis$^{53}$, 
A.~Richards$^{53}$, 
T.~Savidge$^{53}$, 
I.~Sepp$^{53}$, 
A.~Shires$^{53}$, 
D.~Websdale$^{53}$, 
M.~Williams$^{53}$\newline{\it
$ ^{53}$Imperial College London, London, United Kingdom}\\[2ex]
R.B.~Appleby$^{54}$, 
R.J.~Barlow$^{54}$, 
T.~Bird$^{54}$, 
P.M.~Bj\o rnstad$^{54}$, 
D.~Brett$^{54}$, 
J.~Harrison$^{54}$, 
G.~Lafferty$^{54}$, 
G.~McGregor$^{54}$, 
D.~Moran$^{54}$, 
C.~Parkes$^{54}$, 
M.~Smith$^{54}$, 
A.D.~Webber$^{54}$\newline{\it
$ ^{54}$School of Physics and Astronomy, University of Manchester, Manchester, United Kingdom}\\[2ex]
M.~Brock$^{55}$, 
M.~Charles$^{55}$, 
N.~Harnew$^{55}$, 
J.J.~John$^{55}$, 
M.~John$^{55}$, 
S.~Malde$^{55}$, 
A.~Nomerotski$^{55,38}$, 
A.~Powell$^{55}$, 
C.~Thomas$^{55}$, 
S.~Topp-Joergensen$^{55}$, 
G.~Wilkinson$^{55}$\newline{\it
$ ^{55}$Department of Physics, University of Oxford, Oxford, United Kingdom}\\[2ex]
B.~Meadows$^{56}$, 
M.D.~Sokoloff$^{56}$\newline{\it
$ ^{56}$University of Cincinnati, Cincinnati, OH, United States}\\[2ex]
M.~Artuso$^{57,38}$, 
S.~Blusk$^{57}$, 
A.~Borgia$^{57}$, 
T.~Britton$^{57}$, 
J.~Garofoli$^{57}$, 
B.~Gui$^{57}$, 
C.~Hadjivasiliou$^{57}$, 
R.~Mountain$^{57}$, 
B.K.~Pal$^{57}$, 
A.~Phan$^{57}$, 
W.~Qian$^{57}$, 
T.~Skwarnicki$^{57}$, 
S.~Stone$^{57,38}$, 
J.~Wang$^{57}$, 
Z.~Xing$^{57}$, 
L.~Zhang$^{57}$.\newline{\it
$ ^{57}$Syracuse University, Syracuse, NY, United States}\\[2ex]
\bigskip

{\footnotesize \it
\bigskip
$ ^{a}$P.N. Lebedev Physical Institute, Russian Academy of Science (LPI RAS), Moscow, Russia\\
$ ^{b}$Universit\`{a} di Bari, Bari, Italy\\
$ ^{c}$Universit\`{a} di Bologna, Bologna, Italy\\
$ ^{d}$Universit\`{a} di Cagliari, Cagliari, Italy\\
$ ^{e}$Universit\`{a} di Ferrara, Ferrara, Italy\\
$ ^{f}$Universit\`{a} di Firenze, Firenze, Italy\\
$ ^{g}$Universit\`{a} di Urbino, Urbino, Italy\\
$ ^{h}$Universit\`{a} di Modena e Reggio Emilia, Modena, Italy\\
$ ^{i}$Universit\`{a} di Genova, Genova, Italy\\
$ ^{j}$Universit\`{a} di Milano Bicocca, Milano, Italy\\
$ ^{k}$Universit\`{a} di Roma Tor Vergata, Roma, Italy\\
$ ^{l}$Universit\`{a} di Roma La Sapienza, Roma, Italy\\
$ ^{m}$Universit\`{a} della Basilicata, Potenza, Italy\\
$ ^{n}$LIFAELS, La Salle, Universitat Ramon Llull, Barcelona, Spain\\
$ ^{o}$Port d'Informaci\'{o} Cient\'{i}fica (PIC), Barcelona, Spain\\
$ ^{p}$Hanoi University of Science, Hanoi, Viet Nam\\
}
\end{flushleft}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> LHCb_authorlist_sorted_along_institutes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\centerline{\large\bf LHCb collaboration}
\begin{flushleft}
\small
I.~Bediaga$^{}$, 
J.M.~De~Miranda$^{}$, 
P.~Diniz~Batista$^{}$, 
F.~Ferreira~Rodrigues$^{}$, 
A.~Massafferri$^{}$, 
I.~Nasteva$^{}$, 
A.C.~dos~Reis$^{}$\newline{\it
$ ^{1}$Centro Brasileiro de Pesquisas F\'{i}sicas (CBPF), Rio de Janeiro, Brazil}\\[2ex]
S.~Amato$^{}$, 
K.~Carvalho~Akiba$^{}$, 
L.~De~Paula$^{}$, 
O.~Francisco$^{}$, 
M.~Gandelman$^{}$, 
A.~Gomes$^{}$, 
J.H.~Lopes$^{}$, 
D.~Martins~Tostes$^{}$, 
J.M.~Otalora~Goicochea$^{}$, 
E.~Polycarpo$^{}$, 
M.S.~Rangel$^{}$, 
B.~Souza~De~Paula$^{}$, 
D.~Vieira$^{}$\newline{\it
$ ^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil}\\[2ex]
C.~Baesso$^{}$, 
C.~G\"{o}bel$^{}$, 
J.~Molina~Rodriguez$^{}$\newline{\it
$ ^{3}$Pontif\'{i}cia Universidade Cat\'{o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil}\\[2ex]
P.~Chen$^{39}$, 
Y.~Gao$^{}$, 
G.~Gong$^{}$, 
H.~Gong$^{}$, 
F.~Jing$^{}$, 
Y.~Li$^{}$, 
B.~Liu$^{}$, 
H.~Lu$^{}$, 
B.~Shao$^{}$, 
S.~Wu$^{}$, 
T.~Xue$^{}$, 
Z.~Yang$^{}$, 
X.~Yuan$^{}$, 
M.~Zeng$^{}$, 
F.~Zhang$^{}$, 
Y.~Zhang$^{}$, 
L.~Zhong$^{}$\newline{\it
$ ^{4}$Center for High Energy Physics, Tsinghua University, Beijing, China}\\[2ex]
I.~De~Bonis$^{}$, 
D.~Decamp$^{}$, 
C.~Drancourt$^{}$, 
Ph.~Ghez$^{}$, 
P.~Hopchev$^{}$, 
J.-P.~Lees$^{}$, 
I.V.~Machikhiliyan$^{31}$, 
M.-N.~Minard$^{}$, 
B.~Pietrzyk$^{}$, 
W.~Qian$^{}$, 
S.~T'Jampens$^{}$, 
V.~Tisserand$^{}$, 
E.~Tournefier$^{53}$, 
G.~Vouters$^{}$\newline{\it
$ ^{5}$LAPP, Universit\'{e} de Savoie, CNRS/IN2P3, Annecy-Le-Vieux, France}\\[2ex]
Z.~Ajaltouni$^{}$, 
H.~Chanal$^{}$, 
E.~Cogneras$^{}$, 
O.~Deschamps$^{}$, 
I.~El~Rifai$^{}$, 
P.~Henrard$^{}$, 
M.~Hoballah$^{}$, 
R.~Lef\`{e}vre$^{}$, 
L.~Li~Gioi$^{}$, 
S.~Monteil$^{}$, 
V.~Niess$^{}$, 
P.~Perret$^{}$, 
D.A.~Roa~Romero$^{}$, 
K.~Sobczak$^{}$\newline{\it
$ ^{6}$Clermont Universit\'{e}, Universit\'{e} Blaise Pascal, CNRS/IN2P3, LPC, Clermont-Ferrand, France}\\[2ex]
C.~Adrover$^{}$, 
E.~Aslanides$^{}$, 
J.-P.~Cachemiche$^{}$, 
J.~Cogan$^{}$, 
P.-Y.~Duval$^{}$, 
F.~Hachon$^{}$, 
R.~Le~Gac$^{}$, 
O.~Leroy$^{}$, 
G.~Mancinelli$^{}$, 
E.~Maurice$^{}$, 
M.~Perrin-Terrin$^{}$, 
F.~Rethore$^{}$, 
M.~Sapunov$^{}$, 
J.~Serrano$^{}$, 
A.~Tsaregorodtsev$^{}$\newline{\it
$ ^{7}$CPPM, Aix-Marseille Universit\'{e}, CNRS/IN2P3, Marseille, France}\\[2ex]
S.~Barsuk$^{}$, 
C.~Beigbeder-Beau$^{}$, 
T.~Cac\'{e}r\`{e}s$^{}$, 
O.~Callot$^{}$, 
D.~Charlet$^{}$, 
O.~Duarte$^{}$, 
J.~He$^{}$, 
O.~Kochebina$^{}$, 
J.~Lefran\c{c}ois$^{}$, 
F.~Machefert$^{}$, 
A.~Mart\'{i}n~S\'{a}nchez$^{}$, 
M.~Nicol$^{}$, 
P.~Robbe$^{}$, 
M.-H.~Schune$^{}$, 
M.~Teklishyn$^{}$, 
V.~Tocut$^{}$, 
B.~Viaud$^{}$\newline{\it
$ ^{8}$LAL, Universit\'{e} Paris-Sud, CNRS/IN2P3, Orsay, France}\\[2ex]
E.~Ben-Haim$^{}$, 
M.~Benayoun$^{}$, 
P.~David$^{}$, 
L.~Del~Buono$^{}$, 
A.~Martens$^{}$, 
F.~Polci$^{}$\newline{\it
$ ^{9}$LPNHE, Universit\'{e} Pierre et Marie Curie, Universit\'{e} Paris Diderot, CNRS/IN2P3, Paris, France}\\[2ex]
T.~Brambach$^{}$, 
Ch.~Cauet$^{}$, 
M.~Deckenhoff$^{}$, 
M.~Domke$^{}$, 
R.~Ekelhof$^{}$, 
M.~Kaballo$^{}$, 
F.~Kruse$^{}$, 
K.~Rudloff$^{}$, 
S.~Schleich$^{}$, 
M.~Schlupp$^{}$, 
B.~Spaan$^{}$, 
S.~Swientek$^{}$, 
K.~Warda$^{}$, 
J.~Wishahi$^{}$\newline{\it
$ ^{10}$Fakult\"{a}t Physik, Technische Universit\"{a}t Dortmund, Dortmund, Germany}\\[2ex]
O.~Aquines~Gutierrez$^{}$, 
M.~Britsch$^{}$, 
C.~F\"{o}hr$^{}$, 
M.~Fontana$^{}$, 
H.~Fuchs$^{}$, 
W.~Hofmann$^{}$, 
T.~Kihm$^{}$, 
D.~Popov$^{}$, 
M.~Schmelling$^{}$, 
D.~Volyanskyy$^{}$, 
H.~Voss$^{}$, 
M.~Zavertyaev$^{a}$\newline{\it
$ ^{11}$Max-Planck-Institut f\"{u}r Kernphysik (MPIK), Heidelberg, Germany}\\[2ex]
A.~Adametz$^{}$, 
S.~Bachmann$^{}$, 
A.~Bien$^{}$, 
J.~Blouw$^{}$, 
A.~Di~Canto$^{}$, 
F.~Dordei$^{}$, 
C.~F\"{a}rber$^{}$, 
E.~Gersabeck$^{}$, 
S.~Hansmann-Menzemer$^{}$, 
A.~Jaeger$^{}$, 
K.~Kreplin$^{}$, 
G.~Krocker$^{}$, 
C.~Linn$^{}$, 
J.~Marks$^{}$, 
M.~Meissner$^{}$, 
T.~Nikodem$^{}$, 
P.~Seyfert$^{}$, 
S.~Stahl$^{}$, 
J.~van~Tilburg$^{}$, 
U.~Uwer$^{}$, 
S.~Wandernoth$^{}$, 
D.~Wiedner$^{}$, 
A.~Zhelezov$^{}$\newline{\it
$ ^{12}$Physikalisches Institut, Ruprecht-Karls-Universit\"{a}t Heidelberg, Heidelberg, Germany}\\[2ex]
O.~Gr\"{u}nberg$^{}$, 
T.~Hartmann$^{}$, 
C.~Vo\ss$^{}$, 
R.~Waldi$^{}$\newline{\it
$ ^{13}$Institut f\"{u}r Physik, Universit\"{a}t Rostock, Rostock, Germany}\\[2ex]
S.~Bifani$^{}$, 
S.~Farry$^{}$, 
P.~Ilten$^{}$, 
T.~Kechadi$^{}$, 
R.~McNulty$^{}$, 
R.~Wallace$^{}$, 
W.C.~Zhang$^{}$\newline{\it
$ ^{14}$School of Physics, University College Dublin, Dublin, Ireland}\\[2ex]
D.A.~Milanes$^{}$, 
A.~Palano$^{b}$\newline{\it
$ ^{15}$Sezione INFN di Bari, Bari, Italy}\\[2ex]
A.~Carbone$^{c}$, 
I.~D'Antone$^{}$, 
D.~Derkach$^{}$, 
A.~Falabella$^{e}$, 
D.~Galli$^{c}$, 
I.~Lax$^{}$, 
U.~Marconi$^{}$, 
S.~Perazzini$^{c}$, 
V.~Vagnoni$^{}$, 
G.~Valenti$^{}$, 
M.~Zangoli$^{}$\newline{\it
$ ^{16}$Sezione INFN di Bologna, Bologna, Italy}\\[2ex]
W.~Bonivento$^{}$, 
S.~Cadeddu$^{}$, 
A.~Cardini$^{}$, 
A.~Contu$^{55}$, 
C.~Deplano$^{}$, 
A.~Lai$^{}$, 
G.~Manca$^{d}$, 
R.~Oldeman$^{d,38}$, 
B.~Saitta$^{d}$\newline{\it
$ ^{17}$Sezione INFN di Cagliari, Cagliari, Italy}\\[2ex]
W.~Baldini$^{}$, 
C.~Bozzi$^{}$, 
F.~Evangelisti$^{}$, 
L.~Landi$^{e}$, 
A.~Mazurov$^{33,38,e}$, 
M.~Savrie$^{e}$, 
S.~Squerzanti$^{}$, 
S.~Vecchi$^{}$\newline{\it
$ ^{18}$Sezione INFN di Ferrara, Ferrara, Italy}\\[2ex]
L.~Anderlini$^{f}$, 
A.~Bizzeti$^{h}$, 
M.~Frosini$^{f}$, 
G.~Graziani$^{}$, 
G.~Passaleva$^{}$, 
M.~Veltri$^{g}$\newline{\it
$ ^{19}$Sezione INFN di Firenze, Firenze, Italy}\\[2ex]
M.~Anelli$^{}$, 
F.~Archilli$^{38}$, 
G.~Bencivenni$^{}$, 
P.~Campana$^{38}$, 
P.~Ciambrone$^{}$, 
P.~De~Simone$^{}$, 
G.~Felici$^{}$, 
G.~Lanfranchi$^{38}$, 
M.~Palutan$^{}$, 
A.~Saputi$^{}$, 
A.~Sarti$^{l}$, 
B.~Sciascia$^{}$, 
A.~Sciubba$^{l}$, 
F.~Soomro$^{38}$\newline{\it
$ ^{20}$Laboratori Nazionali dell'INFN di Frascati, Frascati, Italy}\\[2ex]
R.~Cardinale$^{i}$, 
F.~Fontanelli$^{i}$, 
C.~Patrignani$^{i}$, 
A.~Petrolini$^{i}$\newline{\it
$ ^{21}$Sezione INFN di Genova, Genova, Italy}\\[2ex]
M.~Calvi$^{j}$, 
S.~Furcas$^{}$, 
A.~Giachero$^{}$, 
C.~Gotti$^{}$, 
B.~Khanji$^{}$, 
M.~Kucharczyk$^{26,j}$, 
J.~von~Loeben$^{}$, 
M.~Maino$^{}$, 
C.~Matteuzzi$^{}$, 
D.L.~Perego$^{j}$, 
G.~Pessina$^{}$\newline{\it
$ ^{22}$Sezione INFN di Milano Bicocca, Milano, Italy}\\[2ex]
G.~Carboni$^{k}$, 
E.~Santovetti$^{k}$, 
A.~Satta$^{}$\newline{\it
$ ^{23}$Sezione INFN di Roma Tor Vergata, Roma, Italy}\\[2ex]
A.A.~Alves~Jr$^{}$, 
G.~Auriemma$^{m}$, 
V.~Bocci$^{}$, 
G.~Martellotti$^{}$, 
G.~Penso$^{l}$, 
D.~Pinci$^{}$, 
G.~Sabatino$^{k}$, 
R.~Santacesaria$^{}$, 
C.~Satriano$^{m}$\newline{\it
$ ^{24}$Sezione INFN di Roma La Sapienza, Roma, Italy}\\[2ex]
S.~Nisar$^{}$\newline{\it
$ ^{25}$Institute of Information Technology, COMSATS, Lahore, Pakistan}\\[2ex]
M.~Chrzaszcz~$^{}$, 
A.~Dziurda$^{}$, 
T.~Lesiak$^{}$, 
P.~Morawski$^{}$, 
G.~Polok$^{}$, 
M.~Witek$^{}$\newline{\it
$ ^{26}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak\'{o}w, Poland}\\[2ex]
B.~Muryn$^{}$, 
A.~Oblakowska-Mucha$^{}$, 
K.~Senderowska$^{}$, 
T.~Szumlak$^{}$\newline{\it
$ ^{27}$AGH University of Science and Technology, Krak\'{o}w, Poland}\\[2ex]
Z.~Guzik$^{}$, 
A.~Nawrot$^{}$, 
M.~Szczekowski$^{}$, 
A.~Ukleja$^{}$\newline{\it
$ ^{28}$National Center for Nuclear Research (NCBJ), Warsaw, Poland}\\[2ex]
I.~Burducea$^{}$, 
C.~Coca$^{}$, 
M.~Dogaru$^{}$, 
A.~Grecu$^{}$, 
F.~Maciuc$^{}$, 
R.~Muresan$^{}$, 
M.~Orlandea$^{}$, 
C.~Pavel-Nicorescu$^{}$, 
B.~Popovici$^{}$, 
S.~Stoica$^{}$, 
M.~Straticiuc$^{}$, 
E.~Teodorescu$^{}$\newline{\it
$ ^{29}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania}\\[2ex]
G.~Alkhazov$^{}$, 
B.~Bochin$^{}$, 
N.~Bondar$^{}$, 
A.~Dzyuba$^{}$, 
S.~Gets$^{}$, 
V.~Golovtsov$^{}$, 
A.~Kashchuk$^{}$, 
O.~Maev$^{38}$, 
M.~Matveev$^{}$, 
N.~Sagidova$^{}$, 
Y.~Shcheglov$^{}$, 
S.~Volkov$^{}$, 
A.~Vorobyev$^{}$\newline{\it
$ ^{30}$Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia}\\[2ex]
S.~Belogurov$^{}$, 
I.~Belyaev$^{}$, 
V.~Egorychev$^{}$, 
D.~Golubkov$^{}$, 
T.~Kvaratskheliya$^{38}$, 
A.~Semennikov$^{}$, 
P.~Shatalov$^{}$, 
V.~Shevchenko$^{}$\newline{\it
$ ^{31}$Institute of Theoretical and Experimental Physics (ITEP), Moscow, Russia}\\[2ex]
A.~Berezhnoy$^{}$, 
G.~Bogdanova$^{}$, 
M.~Korolev$^{}$, 
A.~Leflat$^{38}$, 
N.~Nikitin$^{}$, 
V.~Volkov$^{}$, 
E.~Zverev$^{}$\newline{\it
$ ^{32}$Institute of Nuclear Physics, Moscow State University (SINP MSU), Moscow, Russia}\\[2ex]
S.~Filippov$^{}$, 
E.~Gushchin$^{}$, 
O.~Karavichev$^{}$, 
L.~Kravchuk$^{}$, 
Y.~Kudenko$^{}$, 
S.~Laptev$^{}$, 
A.~Tikhonov$^{}$\newline{\it
$ ^{33}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAN), Moscow, Russia}\\[2ex]
A.~Bobrov$^{}$, 
A.~Bondar$^{}$, 
S.~Eidelman$^{}$, 
P.~Krokovny$^{}$, 
V.~Kudryavtsev$^{}$, 
L.~Shekhtman$^{}$, 
V.~Vorobyev$^{}$\newline{\it
$ ^{34}$Budker Institute of Nuclear Physics (SB RAS) and Novosibirsk State University, Novosibirsk, Russia}\\[2ex]
A.~Artamonov~$^{}$, 
K.~Belous$^{}$, 
R.~Dzhelyadin$^{}$, 
Yu.~Guz$^{}$, 
A.~Likhoded$^{}$, 
A.~Novoselov$^{}$, 
V.~Obraztsov$^{}$, 
A.~Ostankov$^{}$, 
V.~Romanovsky$^{}$, 
M.~Shapkin$^{}$, 
O.~Stenyakin$^{}$, 
O.~Yushchenko$^{}$\newline{\it
$ ^{35}$Institute for High Energy Physics (IHEP), Protvino, Russia}\\[2ex]
C.~Abellan~Beteta$^{n}$, 
M.~Calvo~Gomez$^{n}$, 
A.~Camboni$^{}$, 
A.~Casajus~Ramo$^{}$, 
A.~Comerma-Montells$^{}$, 
F.~Domingo~Bonal$^{n}$, 
L.~Garrido$^{}$, 
D.~Gascon$^{}$, 
M.~Grabalosa~G\'{a}ndara$^{}$, 
R.~Graciani~Diaz$^{}$, 
E.~Graug\'{e}s$^{}$, 
E.~Lopez~Asamar$^{}$, 
J.~Mauricio$^{}$, 
V.~Mendez-Munoz$^{o}$, 
A.~P\'{e}rez-Calero~Yzquierdo$^{}$, 
E.~Picatoste~Olloqui$^{}$, 
C.~Potterat$^{}$, 
V.~Rives~Molina$^{}$, 
H.~Ruiz$^{}$, 
R.~Vazquez~Gomez$^{}$, 
X.~Vilasis-Cardona$^{n}$\newline{\it
$ ^{36}$Universitat de Barcelona, Barcelona, Spain}\\[2ex]
B.~Adeva$^{}$, 
P.~Alvarez~Cartelle$^{}$, 
X.~Cid~Vidal$^{}$, 
A.~Dosil~Su\'{a}rez$^{}$, 
V.~Fernandez~Albor$^{}$, 
A.~Gallas~Torreira$^{}$, 
J.A.~Hernando~Morata$^{}$, 
D.~Martinez~Santos$^{}$, 
A.~Pazos~Alvarez$^{}$, 
E.~Perez~Trigo$^{}$, 
M.~Plo~Casasus$^{}$, 
P.~Rodriguez~Perez$^{}$, 
A.~Romero~Vidal$^{}$, 
J.J.~Saborido~Silva$^{}$, 
B.~Sanmartin~Sedes$^{}$, 
C.~Santamarina~Rios$^{}$, 
M.~Seco$^{}$, 
P.~Vazquez~Regueiro$^{}$\newline{\it
$ ^{37}$Universidad de Santiago de Compostela, Santiago de Compostela, Spain}\\[2ex]
J.~Albrecht$^{}$, 
F.~Alessio$^{}$, 
C.~Barschel$^{}$, 
T.~Blake$^{}$, 
E.~Bonaccorsi$^{}$, 
L.~Brarda$^{}$, 
J.~Buytaert$^{}$, 
M.~Cattaneo$^{}$, 
B.~Chadaj$^{}$, 
Ph.~Charpentier$^{}$, 
M.~Chebbi$^{}$, 
K.~Ciba$^{}$, 
M.~Clemencic$^{}$, 
J.~Closier$^{}$, 
P.~Collins$^{}$, 
B.~Corajod$^{}$, 
G.~Corti$^{}$, 
B.~Couturier$^{}$, 
C.~D'Ambrosio$^{}$, 
G.~Decreuse$^{}$, 
H.~Dijkstra$^{}$, 
R.~Dumps$^{}$, 
M.~Ferro-Luzzi$^{}$, 
C.~Fitzpatrick$^{}$, 
R.~Forty$^{}$, 
C.~Fournier$^{}$, 
M.~Frank$^{}$, 
C.~Frei$^{}$, 
C.~Gaspar$^{}$, 
V.V.~Gligorov$^{}$, 
L.A.~Granado~Cardoso$^{}$, 
T.~Gys$^{}$, 
C.~Haen$^{}$, 
E.~van~Herwijnen$^{}$, 
R.~Jacobsson$^{}$, 
O.~Jamet$^{}$, 
B.~Jost$^{}$, 
M.~Karacson$^{}$, 
T.M.~Karbach$^{}$, 
U.~Kerzel$^{}$, 
R.~Kristic$^{}$, 
D.~Lacarrere$^{}$, 
E.~Lanciotti$^{}$, 
C.~Langenbruch$^{}$, 
R.~Lindner$^{}$, 
G.~Liu$^{}$, 
R.~Matev$^{}$, 
Z.~Mathe$^{}$, 
N.~Neufeld$^{}$, 
J.~Panman$^{}$, 
M.~Pepe~Altarelli$^{}$, 
D.~Piedigrossi$^{}$, 
N.~Rauschmayr$^{}$, 
S.~Roiser$^{}$, 
L.~Roy$^{}$, 
T.~Ruf$^{}$, 
H.~Schindler$^{}$, 
B.~Schmidt$^{}$, 
T.~Schneider$^{}$, 
A.~Schopper$^{}$, 
R.~Schwemmer$^{}$, 
F.~Stagni$^{}$, 
V.K.~Subbiah$^{}$, 
F.~Teubert$^{}$, 
E.~Thomas$^{}$, 
D.~Tonelli$^{}$, 
M.~Ubeda~Garcia$^{}$, 
O.~Ullaland$^{}$, 
M.~Vesterinen$^{}$, 
J.~Wicht$^{}$, 
W.~Witzeling$^{}$, 
K.~Wyllie$^{}$, 
A.~Zvyagin$^{}$\newline{\it
$ ^{38}$European Organization for Nuclear Research (CERN), Geneva, Switzerland}\\[2ex]
Y.~Amhis$^{}$, 
A.~Bay$^{}$, 
F.~Bernard$^{}$, 
F.~Blanc$^{}$, 
J.~Bressieux$^{}$, 
G.A.~Cowan$^{}$, 
H.~Degaudenzi$^{38}$, 
F.~Dupertuis$^{}$, 
V.~Fave$^{}$, 
R.~Frei$^{}$, 
G.~Haefeli$^{}$, 
P.~Jaton$^{}$, 
A.~Keune$^{}$, 
V.~Komarov$^{32}$, 
V.N.~La~Thi$^{}$, 
N.~Lopez-March$^{}$, 
J.~Luisier$^{}$, 
R.~M\"{a}rki$^{}$, 
B.~Muster$^{}$, 
T.~Nakada$^{}$, 
A.D.~Nguyen$^{}$, 
T.D.~Nguyen$^{}$, 
C.~Nguyen-Mau$^{p}$, 
J.~Prisciandaro$^{}$, 
A.~Puig~Navarro$^{}$, 
B.~Rakotomiaramanana$^{}$, 
J.~Rouvinet$^{}$, 
O.~Schneider$^{}$, 
P.~Szczypka$^{38}$, 
S.~Tourneur$^{}$, 
M.T.~Tran$^{}$, 
G.~Veneziano$^{}$\newline{\it
$ ^{39}$Ecole Polytechnique F\'{e}d\'{e}rale de Lausanne (EPFL), Lausanne, Switzerland}\\[2ex]
J.~Anderson$^{}$, 
R.~Bernet$^{}$, 
E.~Bowen$^{}$, 
A.~B\"{u}chler-Germann$^{}$, 
A.~Bursche$^{}$, 
N.~Chiapolini$^{}$, 
M.~De~Cian$^{}$, 
Ch.~Elsasser$^{}$, 
K.~M\"{u}ller$^{}$, 
C.~Salzmann$^{}$, 
S.~Saornil~Gamarra$^{}$, 
N.~Serra$^{}$, 
O.~Steinkamp$^{}$, 
U.~Straumann$^{}$, 
M.~Tobin$^{}$, 
M.~Tresch$^{}$, 
A.~Vollhardt$^{}$\newline{\it
$ ^{40}$Physik-Institut, Universit\"{a}t Z\"{u}rich, Z\"{u}rich, Switzerland}\\[2ex]
R.~Aaij$^{}$, 
S.~Ali$^{}$, 
H.~Band$^{}$, 
Th.~Bauer$^{}$, 
M.~van~Beuzekom$^{}$, 
V.~van~Beveren$^{}$, 
H.~Boer~Rookhuizen$^{}$, 
L.~Ceelie$^{}$, 
V.~Coco$^{}$, 
P.N.Y.~David$^{}$, 
K.~De~Bruyn$^{}$, 
P.~De~Groen$^{}$, 
D.~van~Eijk$^{}$, 
C.~Farinelli$^{}$, 
V.~Gromov$^{}$, 
B.~van~der~Heijden$^{}$, 
V.~Heijne$^{}$, 
W.~Hulsbergen$^{}$, 
E.~Jans$^{}$, 
F.~Jansen$^{}$, 
L.~Jansen$^{}$, 
P.~Jansweijer$^{}$, 
R.~Kluit$^{}$, 
P.~Koppenburg$^{}$, 
A.~Kozlinskiy$^{}$, 
J.~van~Leerdam$^{}$, 
M.~Martinelli$^{}$, 
M.~Merk$^{}$, 
I.~Mous$^{}$, 
B.~Munneke$^{}$, 
S.~Oggero$^{}$, 
M.~van~Overbeek$^{}$, 
A.~Pellegrino$^{}$, 
O.~van~Petten$^{}$, 
E.~Roeland$^{}$, 
K.~de~Roo$^{}$, 
A.~Schimmel$^{}$, 
H.~Schuijlenburg$^{}$, 
T.~Sluijk$^{}$, 
B.~Storaci$^{}$, 
P.~Tsopelas$^{}$, 
N.~Tuning$^{}$, 
W.~Vink$^{}$, 
P.~Wenerke$^{}$, 
L.~Wiggers$^{}$, 
F.~Zappon$^{}$, 
A.~Zwart$^{}$\newline{\it
$ ^{41}$Nikhef National Institute for Subatomic Physics, Amsterdam, The Netherlands}\\[2ex]
J.~van~den~Brand$^{}$, 
F.~Dettori$^{}$, 
T.~Ketel$^{}$, 
R.F.~Koopman$^{}$, 
J.~Kos$^{}$, 
R.W.~Lambert$^{}$, 
F.~Mul$^{}$, 
G.~Raven$^{}$, 
M.~Schiller$^{}$, 
S.~Tolk$^{}$\newline{\it
$ ^{42}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, The Netherlands}\\[2ex]
A.~Dovbnya$^{}$, 
S.~Kandybei$^{}$, 
I.~Raniuk$^{}$, 
I.~Shapoval$^{38}$, 
O.~Shevchenko$^{}$\newline{\it
$ ^{43}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine}\\[2ex]
V.~Iakovenko$^{}$, 
Y.~Nikolaiko$^{}$, 
O.~Okhrimenko$^{}$, 
M.~Pugatch$^{}$, 
V.~Pugatch$^{}$\newline{\it
$ ^{44}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine}\\[2ex]
D.~Elsby$^{}$, 
P.J.W.~Faulkner$^{}$, 
I.R.~Kenyon$^{}$, 
C.~Lazzeroni$^{}$, 
J.~McCarthy$^{}$, 
M.W.~Slater$^{}$, 
N.K.~Watson$^{}$\newline{\it
$ ^{45}$University of Birmingham, Birmingham, United Kingdom}\\[2ex]
M.~Adinolfi$^{}$, 
J.~Benton$^{}$, 
N.H.~Brook$^{}$, 
A.~Cook$^{}$, 
M.~Coombes$^{}$, 
T.~Hampson$^{}$, 
S.T.~Harnew$^{}$, 
J.~Imong$^{}$, 
P.~Naik$^{}$, 
J.H.~Rademacker$^{}$, 
D.~Souza$^{}$, 
J.J.~Velthuis$^{}$, 
D.~Voong$^{}$\newline{\it
$ ^{46}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom}\\[2ex]
W.~Barter$^{}$, 
M.-O.~Bettler$^{}$, 
H.V.~Cliff$^{}$, 
J.~Dickens$^{}$, 
J.~Garra~Tico$^{}$, 
V.~Gibson$^{}$, 
S.~Gregson$^{}$, 
S.C.~Haines$^{}$, 
C.R.~Jones$^{}$, 
N.~Mangiafave$^{}$, 
G.J.~Rogers$^{}$, 
S.~Sigurdsson$^{}$, 
D.R.~Ward$^{}$, 
S.A.~Wotton$^{}$, 
S.~Wright$^{}$\newline{\it
$ ^{47}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom}\\[2ex]
J.J.~Back$^{}$, 
D.~Craik$^{}$, 
D.~Dossett$^{}$, 
T.~Gershon$^{38}$, 
P.F.~Harrison$^{}$, 
M.~Kreps$^{}$, 
T.~Latham$^{}$, 
T.~Pila\v{r}$^{}$, 
A.~Poluektov$^{34}$, 
M.M.~Reid$^{}$, 
R.~Silva~Coutinho$^{}$, 
M.~Whitehead$^{}$, 
M.P.~Williams$^{49}$\newline{\it
$ ^{48}$Department of Physics, University of Warwick, Coventry, United Kingdom}\\[2ex]
S.~Easo$^{38}$, 
R.~Nandakumar$^{}$, 
A.~Papanestis$^{}$, 
G.N.~Patrick$^{}$, 
S.~Ricciardi$^{}$, 
F.F.~Wilson$^{}$\newline{\it
$ ^{49}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom}\\[2ex]
S.~Benson$^{}$, 
H.~Carranza-Mejia$^{}$, 
P.E.L.~Clarke$^{}$, 
R.~Currie$^{}$, 
S.~Eisenhardt$^{}$, 
G.~Fardell$^{}$, 
D.~Lambert$^{}$, 
H.~Luo$^{}$, 
H.~Mejia$^{}$, 
F.~Muheim$^{}$, 
M.~Needham$^{}$, 
S.~Playfer$^{}$, 
A.~Sparkes$^{}$, 
Y.~Xie$^{38}$, 
R.~Young$^{}$\newline{\it
$ ^{50}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom}\\[2ex]
M.~Alexander$^{}$, 
A.~Bates$^{}$, 
J.~Beddow$^{}$, 
L.~Eklund$^{}$, 
D.~Hynds$^{}$, 
A.~Mac~Raighne$^{}$, 
S.~Ogilvy$^{}$, 
M.~Pappagallo$^{}$, 
P.~Sail$^{}$, 
F.J.P.~Soler$^{}$, 
P.~Spradlin$^{}$\newline{\it
$ ^{51}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom}\\[2ex]
A.~Affolder$^{}$, 
T.J.V.~Bowcock$^{}$, 
H.~Brown$^{}$, 
G.~Casse$^{}$, 
S.~Donleavy$^{}$, 
K.~Hennessy$^{}$, 
E.~Hicks$^{}$, 
T.~Huse$^{}$, 
D.~Hutchcroft$^{}$, 
M.~Liles$^{}$, 
G.D.~Patel$^{}$, 
K.~Rinnert$^{}$, 
T.~Shears$^{38}$, 
N.A.~Smith$^{}$\newline{\it
$ ^{52}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom}\\[2ex]
C.~Blanks$^{}$, 
L.~Carson$^{}$, 
G.~Ciezarek$^{}$, 
S.~Cunliffe$^{}$, 
U.~Egede$^{}$, 
A.~Golutvin$^{31,38}$, 
S.~Hall$^{}$, 
P.~Owen$^{}$, 
C.J.~Parkinson$^{}$, 
M.~Patel$^{}$, 
K.~Petridis$^{}$, 
A.~Richards$^{}$, 
T.~Savidge$^{}$, 
P.~Schaack$^{}$, 
I.~Sepp$^{}$, 
A.~Shires$^{}$, 
D.~Websdale$^{}$, 
M.~Williams$^{q}$\newline{\it
$ ^{53}$Imperial College London, London, United Kingdom}\\[2ex]
R.B.~Appleby$^{}$, 
R.J.~Barlow$^{}$, 
T.~Bird$^{}$, 
P.M.~Bj\o rnstad$^{}$, 
S.~Borghi$^{51}$, 
D.~Brett$^{}$, 
S.~De~Capua$^{}$, 
P.~Garosi$^{}$, 
M.~Gersabeck$^{}$, 
J.~Harrison$^{}$, 
C.~Hombach$^{}$, 
G.~Lafferty$^{}$, 
D.~Moran$^{}$, 
C.~Parkes$^{}$, 
E.~Rodrigues$^{51}$, 
M.~Smith$^{}$, 
D.~Urner$^{}$, 
A.D.~Webber$^{}$\newline{\it
$ ^{54}$School of Physics and Astronomy, University of Manchester, Manchester, United Kingdom}\\[2ex]
M.~Charles$^{}$, 
P.~Gandini$^{}$, 
R.~Gauld$^{}$, 
H.~Gordon$^{}$, 
E.~Greening$^{}$, 
N.~Harnew$^{}$, 
D.~Hill$^{}$, 
P.~Hunt$^{}$, 
N.~Hussain$^{}$, 
M.~John$^{}$, 
D.~Johnson$^{}$, 
S.~Malde$^{}$, 
A.~Nomerotski$^{38}$, 
A.~Powell$^{}$, 
S.~Redford$^{}$, 
E.~Smith$^{49}$, 
C.~Thomas$^{}$, 
S.~Topp-Joergensen$^{}$, 
N.~Torr$^{}$, 
G.~Wilkinson$^{}$\newline{\it
$ ^{55}$Department of Physics, University of Oxford, Oxford, United Kingdom}\\[2ex]
R.~Andreassen$^{}$, 
B.~Meadows$^{}$, 
M.D.~Sokoloff$^{}$\newline{\it
$ ^{56}$University of Cincinnati, Cincinnati, OH, United States}\\[2ex]
M.~Artuso$^{}$, 
S.~Blusk$^{}$, 
A.~Borgia$^{}$, 
T.~Britton$^{}$, 
J.~Garofoli$^{}$, 
B.~Gui$^{}$, 
C.~Hadjivasiliou$^{}$, 
R.~Mountain$^{}$, 
B.K.~Pal$^{}$, 
A.~Phan$^{}$, 
T.~Skwarnicki$^{}$, 
S.~Stone$^{}$, 
J.~Wang$^{}$, 
Z.~Xing$^{}$, 
L.~Zhang$^{}$.\newline{\it
$ ^{57}$Syracuse University, Syracuse, NY, United States}\\[2ex]
\bigskip

{\footnotesize \it
\bigskip
$ ^{a}$P.N. Lebedev Physical Institute, Russian Academy of Science (LPI RAS), Moscow, Russia\\
$ ^{b}$Universit\`{a} di Bari, Bari, Italy\\
$ ^{c}$Universit\`{a} di Bologna, Bologna, Italy\\
$ ^{d}$Universit\`{a} di Cagliari, Cagliari, Italy\\
$ ^{e}$Universit\`{a} di Ferrara, Ferrara, Italy\\
$ ^{f}$Universit\`{a} di Firenze, Firenze, Italy\\
$ ^{g}$Universit\`{a} di Urbino, Urbino, Italy\\
$ ^{h}$Universit\`{a} di Modena e Reggio Emilia, Modena, Italy\\
$ ^{i}$Universit\`{a} di Genova, Genova, Italy\\
$ ^{j}$Universit\`{a} di Milano Bicocca, Milano, Italy\\
$ ^{k}$Universit\`{a} di Roma Tor Vergata, Roma, Italy\\
$ ^{l}$Universit\`{a} di Roma La Sapienza, Roma, Italy\\
$ ^{m}$Universit\`{a} della Basilicata, Potenza, Italy\\
$ ^{n}$LIFAELS, La Salle, Universitat Ramon Llull, Barcelona, Spain\\
$ ^{o}$Port d'Informaci\'{o} Cient\'{i}fica (PIC), Barcelona, Spain\\
$ ^{p}$Hanoi University of Science, Hanoi, Viet Nam\\
$ ^{q}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
}
\end{flushleft}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> LHCb_comma_separated_author.tex <==
LHCb collaboration:
R. Aaij, 
C. Abellan Beteta, 
A. Adametz, 
B. Adeva, 
M. Adinolfi, 
C. Adrover, 
A. Affolder, 
Z. Ajaltouni, 
J. Albrecht, 
F. Alessio, 
M. Alexander, 
S. Ali, 
G. Alkhazov, 
P. Alvarez Cartelle, 
A.A. Alves Jr, 
S. Amato, 
Y. Amhis, 
L. Anderlini, 
J. Anderson, 
R. Andreassen, 
M. Anelli, 
R.B. Appleby, 
O. Aquines Gutierrez, 
F. Archilli, 
A. Artamonov , 
M. Artuso, 
E. Aslanides, 
G. Auriemma, 
S. Bachmann, 
J.J. Back, 
C. Baesso, 
W. Baldini, 
H. Band, 
R.J. Barlow, 
C. Barschel, 
S. Barsuk, 
W. Barter, 
A. Bates, 
Th. Bauer, 
A. Bay, 
J. Beddow, 
I. Bediaga, 
C. Beigbeder-Beau, 
S. Belogurov, 
K. Belous, 
I. Belyaev, 
E. Ben-Haim, 
M. Benayoun, 
G. Bencivenni, 
S. Benson, 
J. Benton, 
A. Berezhnoy, 
F. Bernard, 
R. Bernet, 
M.-O. Bettler, 
M. van Beuzekom, 
V. van Beveren, 
A. Bien, 
S. Bifani, 
T. Bird, 
A. Bizzeti, 
P.M. Bj\o rnstad, 
T. Blake, 
F. Blanc, 
C. Blanks, 
J. Blouw, 
S. Blusk, 
A. Bobrov, 
V. Bocci, 
B. Bochin, 
H. Boer Rookhuizen, 
G. Bogdanova, 
E. Bonaccorsi, 
A. Bondar, 
N. Bondar, 
W. Bonivento, 
S. Borghi, 
A. Borgia, 
T.J.V. Bowcock, 
E. Bowen, 
C. Bozzi, 
T. Brambach, 
J. van den Brand, 
L. Brarda, 
J. Bressieux, 
D. Brett, 
M. Britsch, 
T. Britton, 
N.H. Brook, 
H. Brown, 
A. B\"{u}chler-Germann, 
I. Burducea, 
A. Bursche, 
J. Buytaert, 
T. Cac\'{e}r\`{e}s, 
J.-P. Cachemiche, 
S. Cadeddu, 
O. Callot, 
M. Calvi, 
M. Calvo Gomez, 
A. Camboni, 
P. Campana, 
A. Carbone, 
G. Carboni, 
R. Cardinale, 
A. Cardini, 
H. Carranza-Mejia, 
L. Carson, 
K. Carvalho Akiba, 
A. Casajus Ramo, 
G. Casse, 
M. Cattaneo, 
Ch. Cauet, 
L. Ceelie, 
B. Chadaj, 
H. Chanal, 
M. Charles, 
D. Charlet, 
Ph. Charpentier, 
M. Chebbi, 
P. Chen, 
N. Chiapolini, 
M. Chrzaszcz , 
P. Ciambrone, 
K. Ciba, 
X. Cid Vidal, 
G. Ciezarek, 
P.E.L. Clarke, 
M. Clemencic, 
H.V. Cliff, 
J. Closier, 
C. Coca, 
V. Coco, 
J. Cogan, 
E. Cogneras, 
P. Collins, 
A. Comerma-Montells, 
A. Contu, 
A. Cook, 
M. Coombes, 
B. Corajod, 
G. Corti, 
B. Couturier, 
G.A. Cowan, 
D. Craik, 
S. Cunliffe, 
R. Currie, 
C. D'Ambrosio, 
I. D'Antone, 
P. David, 
P.N.Y. David, 
I. De Bonis, 
K. De Bruyn, 
S. De Capua, 
M. De Cian, 
P. De Groen, 
J.M. De Miranda, 
L. De Paula, 
P. De Simone, 
D. Decamp, 
M. Deckenhoff, 
G. Decreuse, 
H. Degaudenzi, 
L. Del Buono, 
C. Deplano, 
D. Derkach, 
O. Deschamps, 
F. Dettori, 
A. Di Canto, 
J. Dickens, 
H. Dijkstra, 
P. Diniz Batista, 
M. Dogaru, 
F. Domingo Bonal, 
M. Domke, 
S. Donleavy, 
F. Dordei, 
A. Dosil Su\'{a}rez, 
D. Dossett, 
A. Dovbnya, 
C. Drancourt, 
O. Duarte, 
R. Dumps, 
F. Dupertuis, 
P.-Y. Duval, 
R. Dzhelyadin, 
A. Dziurda, 
A. Dzyuba, 
S. Easo, 
U. Egede, 
V. Egorychev, 
S. Eidelman, 
D. van Eijk, 
S. Eisenhardt, 
R. Ekelhof, 
L. Eklund, 
I. El Rifai, 
Ch. Elsasser, 
D. Elsby, 
F. Evangelisti, 
A. Falabella, 
C. F\"{a}rber, 
G. Fardell, 
C. Farinelli, 
S. Farry, 
P.J.W. Faulkner, 
V. Fave, 
G. Felici, 
V. Fernandez Albor, 
F. Ferreira Rodrigues, 
M. Ferro-Luzzi, 
S. Filippov, 
C. Fitzpatrick, 
C. F\"{o}hr, 
M. Fontana, 
F. Fontanelli, 
R. Forty, 
C. Fournier, 
O. Francisco, 
M. Frank, 
C. Frei, 
R. Frei, 
M. Frosini, 
H. Fuchs, 
S. Furcas, 
A. Gallas Torreira, 
D. Galli, 
M. Gandelman, 
P. Gandini, 
Y. Gao, 
J. Garofoli, 
P. Garosi, 
J. Garra Tico, 
L. Garrido, 
D. Gascon, 
C. Gaspar, 
R. Gauld, 
E. Gersabeck, 
M. Gersabeck, 
T. Gershon, 
S. Gets, 
Ph. Ghez, 
A. Giachero, 
V. Gibson, 
V.V. Gligorov, 
C. G\"{o}bel, 
V. Golovtsov, 
D. Golubkov, 
A. Golutvin, 
A. Gomes, 
G. Gong, 
H. Gong, 
H. Gordon, 
C. Gotti, 
M. Grabalosa G\'{a}ndara, 
R. Graciani Diaz, 
L.A. Granado Cardoso, 
E. Graug\'{e}s, 
G. Graziani, 
A. Grecu, 
E. Greening, 
S. Gregson, 
V. Gromov, 
O. Gr\"{u}nberg, 
B. Gui, 
E. Gushchin, 
Yu. Guz, 
Z. Guzik, 
T. Gys, 
F. Hachon, 
C. Hadjivasiliou, 
G. Haefeli, 
C. Haen, 
S.C. Haines, 
S. Hall, 
T. Hampson, 
S. Hansmann-Menzemer, 
N. Harnew, 
S.T. Harnew, 
J. Harrison, 
P.F. Harrison, 
T. Hartmann, 
J. He, 
B. van der Heijden, 
V. Heijne, 
K. Hennessy, 
P. Henrard, 
J.A. Hernando Morata, 
E. van Herwijnen, 
E. Hicks, 
D. Hill, 
M. Hoballah, 
W. Hofmann, 
C. Hombach, 
P. Hopchev, 
W. Hulsbergen, 
P. Hunt, 
T. Huse, 
N. Hussain, 
D. Hutchcroft, 
D. Hynds, 
V. Iakovenko, 
P. Ilten, 
J. Imong, 
R. Jacobsson, 
A. Jaeger, 
O. Jamet, 
E. Jans, 
F. Jansen, 
L. Jansen, 
P. Jansweijer, 
P. Jaton, 
F. Jing, 
M. John, 
D. Johnson, 
C.R. Jones, 
B. Jost, 
M. Kaballo, 
S. Kandybei, 
M. Karacson, 
O. Karavichev, 
T.M. Karbach, 
A. Kashchuk, 
T. Kechadi, 
I.R. Kenyon, 
U. Kerzel, 
T. Ketel, 
A. Keune, 
B. Khanji, 
T. Kihm, 
R. Kluit, 
O. Kochebina, 
V. Komarov, 
R.F. Koopman, 
P. Koppenburg, 
M. Korolev, 
J. Kos, 
A. Kozlinskiy, 
L. Kravchuk, 
K. Kreplin, 
M. Kreps, 
R. Kristic, 
G. Krocker, 
P. Krokovny, 
F. Kruse, 
M. Kucharczyk, 
Y. Kudenko, 
V. Kudryavtsev, 
T. Kvaratskheliya, 
V.N. La Thi, 
D. Lacarrere, 
G. Lafferty, 
A. Lai, 
D. Lambert, 
R.W. Lambert, 
E. Lanciotti, 
L. Landi, 
G. Lanfranchi, 
C. Langenbruch, 
S. Laptev, 
T. Latham, 
I. Lax, 
C. Lazzeroni, 
R. Le Gac, 
J. van Leerdam, 
J.-P. Lees, 
R. Lef\`{e}vre, 
A. Leflat, 
J. Lefran\c{c}ois, 
O. Leroy, 
T. Lesiak, 
Y. Li, 
L. Li Gioi, 
A. Likhoded, 
M. Liles, 
R. Lindner, 
C. Linn, 
B. Liu, 
G. Liu, 
J. von Loeben, 
J.H. Lopes, 
E. Lopez Asamar, 
N. Lopez-March, 
H. Lu, 
J. Luisier, 
H. Luo, 
A. Mac Raighne, 
F. Machefert, 
I.V. Machikhiliyan, 
F. Maciuc, 
O. Maev, 
M. Maino, 
S. Malde, 
G. Manca, 
G. Mancinelli, 
N. Mangiafave, 
U. Marconi, 
R. M\"{a}rki, 
J. Marks, 
G. Martellotti, 
A. Martens, 
A. Mart\'{i}n S\'{a}nchez, 
M. Martinelli, 
D. Martinez Santos, 
D. Martins Tostes, 
A. Massafferri, 
R. Matev, 
Z. Mathe, 
C. Matteuzzi, 
M. Matveev, 
E. Maurice, 
J. Mauricio, 
A. Mazurov, 
J. McCarthy, 
R. McNulty, 
B. Meadows, 
M. Meissner, 
H. Mejia, 
V. Mendez-Munoz, 
M. Merk, 
D.A. Milanes, 
M.-N. Minard, 
J. Molina Rodriguez, 
S. Monteil, 
D. Moran, 
P. Morawski, 
R. Mountain, 
I. Mous, 
F. Muheim, 
F. Mul, 
K. M\"{u}ller, 
B. Munneke, 
R. Muresan, 
B. Muryn, 
B. Muster, 
P. Naik, 
T. Nakada, 
R. Nandakumar, 
I. Nasteva, 
A. Nawrot, 
M. Needham, 
N. Neufeld, 
A.D. Nguyen, 
T.D. Nguyen, 
C. Nguyen-Mau, 
M. Nicol, 
V. Niess, 
N. Nikitin, 
T. Nikodem, 
Y. Nikolaiko, 
S. Nisar, 
A. Nomerotski, 
A. Novoselov, 
A. Oblakowska-Mucha, 
V. Obraztsov, 
S. Oggero, 
S. Ogilvy, 
O. Okhrimenko, 
R. Oldeman, 
M. Orlandea, 
A. Ostankov, 
J.M. Otalora Goicochea, 
M. van Overbeek, 
P. Owen, 
B.K. Pal, 
A. Palano, 
M. Palutan, 
J. Panman, 
A. Papanestis, 
M. Pappagallo, 
C. Parkes, 
C.J. Parkinson, 
G. Passaleva, 
G.D. Patel, 
M. Patel, 
G.N. Patrick, 
C. Patrignani, 
C. Pavel-Nicorescu, 
A. Pazos Alvarez, 
A. Pellegrino, 
G. Penso, 
M. Pepe Altarelli, 
S. Perazzini, 
D.L. Perego, 
E. Perez Trigo, 
A. P\'{e}rez-Calero Yzquierdo, 
P. Perret, 
M. Perrin-Terrin, 
G. Pessina, 
K. Petridis, 
A. Petrolini, 
O. van Petten, 
A. Phan, 
E. Picatoste Olloqui, 
D. Piedigrossi, 
B. Pietrzyk, 
T. Pila\v{r}, 
D. Pinci, 
S. Playfer, 
M. Plo Casasus, 
F. Polci, 
G. Polok, 
A. Poluektov, 
E. Polycarpo, 
D. Popov, 
B. Popovici, 
C. Potterat, 
A. Powell, 
J. Prisciandaro, 
M. Pugatch, 
V. Pugatch, 
A. Puig Navarro, 
W. Qian, 
J.H. Rademacker, 
B. Rakotomiaramanana, 
M.S. Rangel, 
I. Raniuk, 
N. Rauschmayr, 
G. Raven, 
S. Redford, 
M.M. Reid, 
A.C. dos Reis, 
F. Rethore, 
S. Ricciardi, 
A. Richards, 
K. Rinnert, 
V. Rives Molina, 
D.A. Roa Romero, 
P. Robbe, 
E. Rodrigues, 
P. Rodriguez Perez, 
E. Roeland, 
G.J. Rogers, 
S. Roiser, 
V. Romanovsky, 
A. Romero Vidal, 
K. de Roo, 
J. Rouvinet, 
L. Roy, 
K. Rudloff, 
T. Ruf, 
H. Ruiz, 
G. Sabatino, 
J.J. Saborido Silva, 
N. Sagidova, 
P. Sail, 
B. Saitta, 
C. Salzmann, 
B. Sanmartin Sedes, 
R. Santacesaria, 
C. Santamarina Rios, 
E. Santovetti, 
S. Saornil Gamarra, 
M. Sapunov, 
A. Saputi, 
A. Sarti, 
C. Satriano, 
A. Satta, 
T. Savidge, 
M. Savrie, 
P. Schaack, 
M. Schiller, 
A. Schimmel, 
H. Schindler, 
S. Schleich, 
M. Schlupp, 
M. Schmelling, 
B. Schmidt, 
O. Schneider, 
T. Schneider, 
A. Schopper, 
H. Schuijlenburg, 
M.-H. Schune, 
R. Schwemmer, 
B. Sciascia, 
A. Sciubba, 
M. Seco, 
A. Semennikov, 
K. Senderowska, 
I. Sepp, 
N. Serra, 
J. Serrano, 
P. Seyfert, 
B. Shao, 
M. Shapkin, 
I. Shapoval, 
P. Shatalov, 
Y. Shcheglov, 
T. Shears, 
L. Shekhtman, 
O. Shevchenko, 
V. Shevchenko, 
A. Shires, 
S. Sigurdsson, 
R. Silva Coutinho, 
T. Skwarnicki, 
M.W. Slater, 
T. Sluijk, 
N.A. Smith, 
E. Smith, 
M. Smith, 
K. Sobczak, 
M.D. Sokoloff, 
F.J.P. Soler, 
F. Soomro, 
D. Souza, 
B. Souza De Paula, 
B. Spaan, 
A. Sparkes, 
P. Spradlin, 
S. Squerzanti, 
F. Stagni, 
S. Stahl, 
O. Steinkamp, 
O. Stenyakin, 
S. Stoica, 
S. Stone, 
B. Storaci, 
M. Straticiuc, 
U. Straumann, 
V.K. Subbiah, 
S. Swientek, 
M. Szczekowski, 
P. Szczypka, 
T. Szumlak, 
S. T'Jampens, 
M. Teklishyn, 
E. Teodorescu, 
F. Teubert, 
C. Thomas, 
E. Thomas, 
A. Tikhonov, 
J. van Tilburg, 
V. Tisserand, 
M. Tobin, 
V. Tocut, 
S. Tolk, 
D. Tonelli, 
S. Topp-Joergensen, 
N. Torr, 
E. Tournefier, 
S. Tourneur, 
M.T. Tran, 
M. Tresch, 
A. Tsaregorodtsev, 
P. Tsopelas, 
N. Tuning, 
M. Ubeda Garcia, 
A. Ukleja, 
O. Ullaland, 
D. Urner, 
U. Uwer, 
V. Vagnoni, 
G. Valenti, 
R. Vazquez Gomez, 
P. Vazquez Regueiro, 
S. Vecchi, 
J.J. Velthuis, 
M. Veltri, 
G. Veneziano, 
M. Vesterinen, 
B. Viaud, 
D. Vieira, 
X. Vilasis-Cardona, 
W. Vink, 
S. Volkov, 
V. Volkov, 
A. Vollhardt, 
D. Volyanskyy, 
D. Voong, 
A. Vorobyev, 
V. Vorobyev, 
C. Vo\ss, 
H. Voss, 
G. Vouters, 
R. Waldi, 
R. Wallace, 
S. Wandernoth, 
J. Wang, 
D.R. Ward, 
K. Warda, 
N.K. Watson, 
A.D. Webber, 
D. Websdale, 
P. Wenerke, 
M. Whitehead, 
J. Wicht, 
D. Wiedner, 
L. Wiggers, 
G. Wilkinson, 
M.P. Williams, 
M. Williams, 
F.F. Wilson, 
J. Wishahi, 
M. Witek, 
W. Witzeling, 
S.A. Wotton, 
S. Wright, 
S. Wu, 
K. Wyllie, 
Y. Xie, 
Z. Xing, 
T. Xue, 
Z. Yang, 
R. Young, 
X. Yuan, 
O. Yushchenko, 
M. Zangoli, 
F. Zappon, 
M. Zavertyaev, 
M. Zeng, 
F. Zhang, 
L. Zhang, 
W.C. Zhang, 
Y. Zhang, 
A. Zhelezov, 
L. Zhong, 
E. Zverev, 
A. Zvyagin, 
A. Zwart


==> charm_theory_defs.tex <==
\usepackage{cancel}

\newcommand{\vckm}{V^{\rm CKM}}
%\newcommand{\beq}{\begin{equation}}
%\newcommand{\eeq}{\end{equation}}
\newcommand{\co}{\mathcal{O}}
\newcommand{\ddbar}{D^0-\overline{D^0}}



\newcommand{\re}[0]{\mathrm{Re}\,}
\newcommand{\im}[0]{\mathrm{Im}\,}
\newcommand{\cH}{\mathcal H}
\newcommand{\cB}{\mathcal B}
\newcommand{\cA}{\mathcal A}
%\newcommand{\be}{\begin{equation}}
%\newcommand{\ee}{\end{equation}}
%\newcommand{\bea}{\begin{eqnarray}}
%\newcommand{\eea}{\end{eqnarray}}
\newcommand{\lsim}{\stackrel{<}{_\sim}}
\newcommand{\gsim}{\stackrel{>}{_\sim}}


%\newcommand{\slashed}{\slash \hspace{-0.19cm}}
\newcommand {\E}[1]{\times 10^{#1}}
\newcommand {\e}[1]{\mathrm{~#1}}
%\newcommand{\re}[0]{\mathrm{Re}\,}
%\newcommand{\im}[0]{\mathrm{Im}\,}
%\newcommand{\cH}{\mathcal H}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\dd}[0]{\mathrm{d}}
%\newcommand{\be}{\begin{equation}}
%\newcommand{\ee}{\end{equation}}
\newcommand{\no}{\nonumber}
%\newcommand{\bea}{\begin{eqnarray}}
%\newcommand{\eea}{\end{eqnarray}}
%\newcommand{\SM}{{\rm SM}}
%\newcommand{\NP}{{\rm NP}}
%\newcommand{\ntree}{{\rm peng}}
%\newcommand{\cB}{\mathcal{B}}


\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\ba{\begin{eqnarray}}
\def\ea{\end{eqnarray}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}

\newcommand{\pk}{|{\bf{\hat p_K}}|}
\newcommand{\tree}{{\rm tree}}
%\newcommand{\SM}{{\rm SM}}
%\newcommand{\NP}{{\rm NP}}
\newcommand{\ntree}{{\rm peng}}
%\newcommand{\lsim}{\stackrel{<}{_\sim}}
%\newcommand{\gsim}{\stackrel{>}{_\sim}}

\newcommand{\op}{{\cal Q}}
\newcommand{\nn}{\nonumber}
\newcommand{\ii}{\mathrm{i}}

\newcommand{\yut}{(Y_u Y_u^\dagger)_{\slashed{\mathrm{tr}}}}
\newcommand{\ydt}{(Y_d Y_d^\dagger)_{\slashed{\mathrm{tr}}}}
\newcommand{\au}{\mathcal{A}_u}
\newcommand{\ad}{\mathcal{A}_d}
\newcommand{\slashed}{\slash \hspace{-0.23cm}}
%\newcommand{\lsim}{\mathrel{\rlap{\lower4pt\hbox{\hskip1pt$\sim$}}
%    \raise1pt\hbox{$<$}}}         %less than or approx. symbol
%\newcommand{\gsim}{\mathrel{\rlap{\lower4pt\hbox{\hskip1pt$\sim$}}
%    \raise1pt\hbox{$>$}}}         %greater than or approx. symbol

\newcommand{\leftrightarrowraised}{\mathrel{\rlap{\lower-0pt\hbox{\hskip1pt$\partial$}}
    \raise6 pt\hbox{$\leftrightarrow$}}}    
    
\newcommand{\deriv}{\stackrel{\leftrightarrow}{\partial}}
\newcommand{\derleft}{\stackrel{\leftarrow}{\partial}}
\newcommand{\derright}{\stackrel{\rightarrow}{\partial}}


==> lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script ./listsymbols

\section{List of all symbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash ux85} & \ux85 & \texttt{\textbackslash cern} & \cern \\
\texttt{\textbackslash lhc} & \lhc & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle & \texttt{\textbackslash aleph} & \aleph \\
\texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal & \texttt{\textbackslash lthree} & \lthree \\
\texttt{\textbackslash lep} & \lep & \texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero \\
\texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cleo} & \cleo & \texttt{\textbackslash uaone} & \uaone \\
\texttt{\textbackslash uatwo} & \uatwo & \texttt{\textbackslash tevatron} & \tevatron &  \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash pu} & \pu & \texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich \\
\texttt{\textbackslash richone} & \richone & \texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker \\
\texttt{\textbackslash intr} & \intr & \texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot \\
\texttt{\textbackslash Tone} & \Tone & \texttt{\textbackslash Ttwo} & \Ttwo & \texttt{\textbackslash Tthree} & \Tthree \\
\texttt{\textbackslash Mone} & \Mone & \texttt{\textbackslash Mtwo} & \Mtwo & \texttt{\textbackslash Mthree} & \Mthree \\
\texttt{\textbackslash Mfour} & \Mfour & \texttt{\textbackslash Mfive} & \Mfive & \texttt{\textbackslash ecal} & \ecal \\
\texttt{\textbackslash spd} & \spd & \texttt{\textbackslash presh} & \presh & \texttt{\textbackslash hcal} & \hcal \\
\texttt{\textbackslash bcm} & \bcm & \texttt{\textbackslash ode} & \ode & \texttt{\textbackslash daq} & \daq \\
\texttt{\textbackslash tfc} & \tfc & \texttt{\textbackslash ecs} & \ecs & \texttt{\textbackslash lone} & \lone \\
\texttt{\textbackslash hlt} & \hlt & \texttt{\textbackslash hltone} & \hltone & \texttt{\textbackslash hlttwo} & \hlttwo \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash epem} & \epem & \texttt{\textbackslash ee} & \ee \\
\texttt{\textbackslash mmu} & \mmu & \texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun \\
\texttt{\textbackslash mumu} & \mumu & \texttt{\textbackslash mtau} & \mtau & \texttt{\textbackslash taup} & \taup \\
\texttt{\textbackslash taum} & \taum & \texttt{\textbackslash tautau} & \tautau & \texttt{\textbackslash ellm} & \ellm \\
\texttt{\textbackslash ellp} & \ellp & \texttt{\textbackslash ellell} & \ellell & \texttt{\textbackslash neu} & \neu \\
\texttt{\textbackslash neub} & \neub & \texttt{\textbackslash nuenueb} & \nuenueb & \texttt{\textbackslash neue} & \neue \\
\texttt{\textbackslash neueb} & \neueb & \texttt{\textbackslash neueneueb} & \neueneueb & \texttt{\textbackslash neum} & \neum \\
\texttt{\textbackslash neumb} & \neumb & \texttt{\textbackslash neumneumb} & \neumneumb & \texttt{\textbackslash neut} & \neut \\
\texttt{\textbackslash neutb} & \neutb & \texttt{\textbackslash neutneutb} & \neutneutb & \texttt{\textbackslash neul} & \neul \\
\texttt{\textbackslash neulb} & \neulb & \texttt{\textbackslash neulneulb} & \neulneulb &  \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz & \texttt{\textbackslash pizs} & \pizs \\
\texttt{\textbackslash ppz} & \ppz & \texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim \\
\texttt{\textbackslash pipi} & \pipi & \texttt{\textbackslash pipm} & \pipm & \texttt{\textbackslash pimp} & \pimp \\
\texttt{\textbackslash kaon} & \kaon & \texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash KzKzb} & \KzKzb & \texttt{\textbackslash Kp} & \Kp \\
\texttt{\textbackslash Km} & \Km & \texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp \\
\texttt{\textbackslash KpKm} & \KpKm & \texttt{\textbackslash KS} & \KS & \texttt{\textbackslash KL} & \KL \\
\texttt{\textbackslash Kstarz} & \Kstarz & \texttt{\textbackslash Kstarzb} & \Kstarzb & \texttt{\textbackslash Kstar} & \Kstar \\
\texttt{\textbackslash Kstarb} & \Kstarb & \texttt{\textbackslash Kstarp} & \Kstarp & \texttt{\textbackslash Kstarm} & \Kstarm \\
\texttt{\textbackslash Kstarpm} & \Kstarpm & \texttt{\textbackslash Kstarmp} & \Kstarmp & \texttt{\textbackslash etapr} & \etapr \\
\end{tabular*}

\subsubsection{Heavy mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db & \texttt{\textbackslash Dz} & \Dz \\
\texttt{\textbackslash Dzb} & \Dzb & \texttt{\textbackslash DzDzb} & \DzDzb & \texttt{\textbackslash Dp} & \Dp \\
\texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm & \texttt{\textbackslash Dmp} & \Dmp \\
\texttt{\textbackslash DpDm} & \DpDm & \texttt{\textbackslash Dstar} & \Dstar & \texttt{\textbackslash Dstarb} & \Dstarb \\
\texttt{\textbackslash Dstarz} & \Dstarz & \texttt{\textbackslash Dstarzb} & \Dstarzb & \texttt{\textbackslash Dstarp} & \Dstarp \\
\texttt{\textbackslash Dstarm} & \Dstarm & \texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp \\
\texttt{\textbackslash Ds} & \Ds & \texttt{\textbackslash Dsp} & \Dsp & \texttt{\textbackslash Dsm} & \Dsm \\
\texttt{\textbackslash Dspm} & \Dspm & \texttt{\textbackslash Dss} & \Dss & \texttt{\textbackslash Dssp} & \Dssp \\
\texttt{\textbackslash Dssm} & \Dssm & \texttt{\textbackslash Dsspm} & \Dsspm & \texttt{\textbackslash B} & \B \\
\texttt{\textbackslash Bb} & \Bb & \texttt{\textbackslash BBbar} & \BBbar & \texttt{\textbackslash Bz} & \Bz \\
\texttt{\textbackslash Bzb} & \Bzb & \texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub \\
\texttt{\textbackslash Bp} & \Bp & \texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm \\
\texttt{\textbackslash Bmp} & \Bmp & \texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bs} & \Bs \\
\texttt{\textbackslash Bsb} & \Bsb & \texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash Bc} & \Bc \\
\texttt{\textbackslash Bcp} & \Bcp & \texttt{\textbackslash Bcm} & \Bcm & \texttt{\textbackslash Bcpm} & \Bcpm \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash chiczero} & \chiczero & \texttt{\textbackslash chicone} & \chicone \\
\texttt{\textbackslash chictwo} & \chictwo & \texttt{\textbackslash OneS} & \OneS & \texttt{\textbackslash TwoS} & \TwoS \\
\texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS & \texttt{\textbackslash FiveS} & \FiveS \\
\texttt{\textbackslash chic} & \chic &  \\
\end{tabular*}

\subsubsection{Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash L} & \L \\
\texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash Lambdares} & \Lambdares & \texttt{\textbackslash Lambdaresbar} & \Lambdaresbar \\
\texttt{\textbackslash Sigmares} & \Sigmares & \texttt{\textbackslash Sigmaresbar} & \Sigmaresbar & \texttt{\textbackslash Omegares} & \Omegares \\
\texttt{\textbackslash Omegaresbar} & \Omegaresbar & \texttt{\textbackslash Lb} & \Lb & \texttt{\textbackslash Lbbar} & \Lbbar \\
\texttt{\textbackslash Lc} & \Lc & \texttt{\textbackslash Lcbar} & \Lcbar &  \\
\end{tabular*}

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BRvis} & \BRvis & \texttt{\textbackslash BR} & \BR \\
\texttt{\textbackslash decay[2] \textbackslash decay\{\Pa\}\{\Pb \Pc\}} & \decay{\Pa}{\Pb \Pc} & \texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar & \texttt{\textbackslash Vud} & \Vud \\
\texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd & \texttt{\textbackslash Vus} & \Vus \\
\texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts & \texttt{\textbackslash Vub} & \Vub \\
\texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb &  \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash kpi} & \kpi & \texttt{\textbackslash kk} & \kk \\
\texttt{\textbackslash dkpi} & \dkpi & \texttt{\textbackslash dkk} & \dkk & \texttt{\textbackslash dkpicf} & \dkpicf \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsection{Units}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash unit[1] \textbackslash unit\{kg\}} & \unit{kg} &  \\
\end{tabular*}

\subsubsection{Energy and momentum}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash gevc} & \gevc \\
\texttt{\textbackslash mevc} & \mevc & \texttt{\textbackslash gevcc} & \gevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc \\
\texttt{\textbackslash mevcc} & \mevcc &  \\
\end{tabular*}

\subsubsection{Distance and area}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash cm} & \cm \\
\texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm & \texttt{\textbackslash mma} & \mma \\
\texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma & \texttt{\textbackslash nm} & \nm \\
\texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn & \texttt{\textbackslash barnhyph} & \barnhyph \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash mbarnhyph} & \mbarnhyph \\
\texttt{\textbackslash nb} & \nb & \texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb \\
\texttt{\textbackslash invpb} & \invpb & \texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash yr} & \yr & \texttt{\textbackslash hr} & \hr \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst &  \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash deriv} & \deriv \\
\texttt{\textbackslash gsim} & \gsim & \texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} \\
\texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} & \texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag \\
\texttt{\textbackslash PDF} & \PDF &  \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash et} & \et & \texttt{\textbackslash dpp} & \dpp \\
\texttt{\textbackslash dedx} & \dedx &  \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mphi} & \mphi & \texttt{\textbackslash mtheta} & \mtheta & \texttt{\textbackslash ctheta} & \ctheta \\
\texttt{\textbackslash stheta} & \stheta & \texttt{\textbackslash ttheta} & \ttheta & \texttt{\textbackslash degrees} & \degrees \\
\texttt{\textbackslash krad} & \krad & \texttt{\textbackslash mrad} & \mrad & \texttt{\textbackslash rad} & \rad \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash evtgen} & \evtgen & \texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash fluka} & \fluka \\
\texttt{\textbackslash tosca} & \tosca & \texttt{\textbackslash ansys} & \ansys & \texttt{\textbackslash spice} & \spice \\
\texttt{\textbackslash garfield} & \garfield & \texttt{\textbackslash geant} & \geant & \texttt{\textbackslash hepmc} & \hepmc \\
\texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash boole} & \boole \\
\texttt{\textbackslash brunel} & \brunel & \texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash erasmus} & \erasmus \\
\texttt{\textbackslash moore} & \moore & \texttt{\textbackslash ganga} & \ganga & \texttt{\textbackslash dirac} & \dirac \\
\texttt{\textbackslash root} & \root & \texttt{\textbackslash roofit} & \roofit & \texttt{\textbackslash pyroot} & \pyroot \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash python} & \python & \texttt{\textbackslash ruby} & \ruby \\
\texttt{\textbackslash fortran} & \fortran & \texttt{\textbackslash svn} & \svn &  \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbytes} & \kbytes & \texttt{\textbackslash kbsps} & \kbsps & \texttt{\textbackslash kbits} & \kbits \\
\texttt{\textbackslash kbsps} & \kbsps & \texttt{\textbackslash mbsps} & \mbsps & \texttt{\textbackslash mbytes} & \mbytes \\
\texttt{\textbackslash mbps} & \mbps & \texttt{\textbackslash mbsps} & \mbsps & \texttt{\textbackslash gbsps} & \gbsps \\
\texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbsps} & \gbsps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbpy} & \tbpy & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\end{tabular*}


